Approximated and User Steerable tSNE for Progressive Visual Analytics

Progressive Visual Analytics aims at improving the interactivity in existing analytics techniques by means of visualization as well as interaction with intermediate results. One key method for data analysis is dimensionality reduction, for example, to produce 2D embeddings that can be visualized and analyzed efficiently. t-Distributed Stochastic Neighbor Embedding (tSNE) is a well-suited technique for the visualization of several high-dimensional data. tSNE can create meaningful intermediate results but suffers from a slow initialization that constrains its application in Progressive Visual Analytics. We introduce a controllable tSNE approximation (A-tSNE), which trades off speed and accuracy, to enable interactive data exploration. We offer real-time visualization techniques, including a density-based solution and a Magic Lens to inspect the degree of approximation. With this feedback, the user can decide on local refinements and steer the approximation level during the analysis. We demonstrate our technique with several datasets, in a real-world research scenario and for the real-time analysis of high-dimensional streams to illustrate its effectiveness for interactive data analysis.

==> charts/computation_time_CIFAR.tex <==

\addplot[black] coordinates{
(100,60)
(150,120)
(200,169)
(250,219)
(300,272)
(400,400)
(500,550)
(1000,1579)
(2000,5362)
(3000,11615)
(4000,20445)
(5000,30941)
(7500,65738)
(10000,114367)
(15000,255195)
(20000,458783)
(30000,989995)
	};\label{plots:plot4}
\addplot[red] coordinates{(100,10)
(150,30)
(200,39)
(250,47)
(300,69)
(400,109)
(500,179)
(1000,460)
(2000,775)
(3000,1248)
(4000,1661)
(5000,2182)
(7500,3243)
(10000,4816)
(15000,7077)
(20000,10101)
(30000,15383)};\label{plots:plot1}
\addplot[green] coordinates{(100,10)
(150,20)
(200,29)
(250,38)
(300,49)
(400,69)
(500,109)
(1000,235)
(2000,496)
(3000,796)
(4000,1084)
(5000,1314)
(7500,1979)
(10000,2986)
(15000,4590)
(20000,6427)
(30000,10047)};\label{plots:plot2}
\addplot[blue] coordinates{(100,10)
(150,10)
(200,19)
(250,29)
(300,30)
(400,49)
(500,50)
(1000,127)
(2000,246)
(3000,409)
(4000,609)
(5000,699)
(7500,1111)
(10000,1664)
(15000,2746)
(20000,3900)
(30000,6618)};\label{plots:plot3}

==> charts/computation_time_NORB.tex <==

\addplot[black] coordinates{
(100,694)
(150,1271)
(200,1542)
(250,1959)
(300,2385)
(400,3569)
(500,4618)
(600,5878)
(700,6853)
(800,8734)
(900,9981)
(1000,12100)
(1500,22154)
(2000,33318)
(2500,50394)
(3000,69470)
(4000,111988)
(5000,157597)
(7500,321346)
(10000,517111)
(15000,1057260)
(20000,1824110)
	};\label{plots:plot4}
\addplot[red] coordinates{
(100,100)
(150,190)
(200,240)
(250,350)
(300,443)
(400,680)
(500,880)
(600,1170)
(700,1515)
(800,1926)
(900,2402)
(1000,2650)
(1500,4161)
(2000,5575)
(2500,7031)
(3000,8612)
(4000,11349)
(5000,14290)
(7500,21396)
(10000,28897)
(15000,44379)
(20000,57367)
};\label{plots:plot1}
\addplot[green] coordinates{(100,60)
(150,110)
(200,200)
(250,261)
(300,337)
(400,492)
(500,701)
(600,840)
(700,980)
(800,1126)
(900,1285)
(1000,1395)
(1500,2138)
(2000,2898)
(2500,3578)
(3000,4634)
(4000,5913)
(5000,7589)
(7500,10858)
(10000,15194)
(15000,23415)
(20000,29980)};\label{plots:plot2}
\addplot[blue] coordinates{(100,40)
(150,90)
(200,114)
(250,142)
(300,162)
(400,224)
(500,282)
(600,322)
(700,381)
(800,431)
(900,438)
(1000,496)
(1500,693)
(2000,952)
(2500,1271)
(3000,1525)
(4000,2000)
(5000,2414)
(7500,3736)
(10000,4946)
(15000,7986)
(20000,10479)};\label{plots:plot3}

==> charts/computation_time_TIMIT.tex <==

\addplot[black] coordinates{
(100,11)
(150,20)
(200,27)
(250,47)
(300,44)
(400,81)
(500,102)
(600,117)
(700,136)
(800,160)
(1000,201)
(1500,323)
(2000,487)
(3000,885)
(5000,1973)
(7500,3777)
(10000,6031)
(15000,12147)
(20000,21117)
(30000,53320)
(50000,179086)
(75000,389911)
(100000,658749)
(150000,1356910)
(200000,2293420)
	};\label{plots:plot4}
\addplot[red] coordinates{
(100,12)
(150,11)
(200,22)
(250,24)
(300,25)
(400,54)
(500,107)
(600,73)
(700,158)
(800,142)
(1000,174)
(1500,269)
(2000,269)
(3000,436)
(5000,656)
(7500,1042)
(10000,1509)
(15000,2268)
(20000,3120)
(30000,5135)
(50000,9290)
(75000,14736)
(100000,19784)
(150000,31253)
(200000,45310)
};\label{plots:plot1}
\addplot[green] coordinates{(100,5)
(150,8)
(200,13)
(250,20)
(300,22)
(400,49)
(500,52)
(600,58)
(700,74)
(800,67)
(1000,100)
(1500,138)
(2000,171)
(3000,272)
(5000,551)
(7500,844)
(10000,1168)
(15000,1754)
(20000,2517)
(30000,4048)
(50000,7236)
(75000,11733)
(100000,16091)
(150000,25509)
(200000,36370)};\label{plots:plot2}
\addplot[blue] coordinates{(100,4)
(150,8)
(200,17)
(250,18)
(300,28)
(400,28)
(500,35)
(600,44)
(700,51)
(800,56)
(1000,79)
(1500,119)
(2000,151)
(3000,263)
(5000,501)
(7500,844)
(10000,1056)
(15000,1698)
(20000,2422)
(30000,3962)
(50000,7073)
(75000,11431)
(100000,15444)
(150000,24785)
(200000,34225)};\label{plots:plot3}

==> charts/exponential_decay.tex <==
\addplot[black] coordinates{(0,1)
(10,1)
(20,1)
(30,1)
(40,1)
(50,1)
(60,1)
(70,1)
(80,1)
(90,1)
(100,1)
(110,1)
(120,1)
(130,1)
(140,1)
(150,0.9999590042)
(160,0.9955341267)
(170,0.9832122612)
(180,0.964755592)
(190,0.9434756572)
(200,0.9199277489)
(210,0.8952883742)
(220,0.8707124552)
(230,0.8465565414)
(240,0.8235969614)
(250,0.8037745467)
(260,0.8324510242)
(270,0.8446756336)
(280,0.8462764583)
(290,0.8447067558)
(300,0.8436161988)
(310,0.8437923526)
(320,0.8452295297)
(330,0.8474901232)
(340,0.8502550033)
(350,0.8531238028)
(360,0.855940908)
(370,0.8589733359)
(380,0.8620330215)
(390,0.8651106745)
(400,0.8680957546)
(410,0.8709518282)
(420,0.8737207425)
(430,0.8763631195)
(440,0.8789250056)
(450,0.8813827011)
(460,0.8837213522)
(470,0.8859677025)
(480,0.8880102626)
(490,0.8900955794)
(500,0.8921363919)
(510,0.8942619022)
(520,0.8962600465)
(530,0.8982333789)
(540,0.9002407701)
(550,0.9022706771)
(560,0.9041523376)
(570,0.9059105575)
(580,0.9075307528)
(590,0.9091498291)
(600,0.9107016107)
(610,0.9121850548)
(620,0.9135100482)
(630,0.9148236566)
(640,0.9160839161)
(650,0.9173042375)
(660,0.9185257706)
(670,0.9197563343)
(680,0.9209309458)
(690,0.922137341)
(700,0.9233700152)
(710,0.9245513619)
(720,0.9257580656)
(730,0.9269082972)
(740,0.9280407478)
(750,0.9290574707)
(760,0.9299808839)
(770,0.9308617425)
(780,0.9318312266)
(790,0.9327040997)
(800,0.9337823687)
(810,0.934679219)
(820,0.9355685627)
(830,0.9366933491)
(840,0.93765948)
(850,0.9388438127)
(860,0.9398915164)
(870,0.9409175178)
(880,0.941919962)
(890,0.9429122193)
(900,0.9438367604)
(910,0.944676725)
(920,0.945633402)
(930,0.9466402065)
(940,0.9474670755)
(950,0.9484929897)
(960,0.9493321535)
(970,0.9504514983)
(980,0.951324241)
(990,0.9521328696)
(1000,0.9528525557)
(1010,0.9534770778)
(1020,0.9542875564)
(1030,0.9550219502)
(1040,0.9560401548)
(1050,0.9568915677)
(1060,0.9576065453)
(1070,0.9582624871)
(1080,0.9588641943)
(1090,0.9595972135)
(1100,0.9603703839)
(1110,0.96106183)
(1120,0.9616057643)
(1130,0.9623336624)
(1140,0.9629178389)
(1150,0.9636511637)
(1160,0.9642978957)
(1170,0.9650437974)
(1180,0.9655483016)
(1190,0.9661498535)
(1200,0.9665829934)
(1210,0.9668657118)
(1220,0.9672774967)
(1230,0.9676629986)
(1240,0.9680623116)
(1250,0.9684147122)
(1260,0.9687476438)
(1270,0.9693081495)
(1280,0.9697891138)
(1290,0.970243326)
(1300,0.9706393342)
(1310,0.9709870775)
(1320,0.9712686085)
(1330,0.9715763258)
(1340,0.9718924195)
(1350,0.972088194)
(1360,0.9722833731)
(1370,0.9724494716)
(1380,0.9727751981)
(1390,0.973011745)
(1400,0.9731728672)
(1410,0.973348712)
(1420,0.9735095769)
(1430,0.9736422279)
(1440,0.973774767)
(1450,0.9739438089)
(1460,0.9739766602)
(1470,0.9741646279)
(1480,0.9743130644)
(1490,0.9744347718)
(1500,0.9745832492)
(1510,0.9746405269)
(1520,0.9747761775)
(1530,0.9749431057)
(1540,0.9751416132)
(1550,0.9752712276)
(1560,0.9754705326)
(1570,0.9756861272)
(1580,0.9758171318)
(1590,0.9761105271)
(1600,0.9762903276)
(1610,0.9764847398)
(1620,0.9767108732)
(1630,0.9769459261)
(1640,0.9770972499)
(1650,0.9773340912)
(1660,0.9775078438)
(1670,0.9777693391)
(1680,0.9779995248)
(1690,0.9782538034)
(1700,0.9783512681)
(1710,0.9786302719)
(1720,0.9788951357)
(1730,0.9789945397)
(1740,0.9791331368)
(1750,0.9792889499)
(1760,0.9794051439)
(1770,0.9795378641)
(1780,0.9797093567)
(1790,0.9799207398)
(1800,0.9800766161)
(1810,0.980241942)
(1820,0.9803441382)
(1830,0.9805817439)
(1840,0.9807718609)
(1850,0.981098494)
(1860,0.9814481863)
(1870,0.9816551524)
(1880,0.9819431877)
(1890,0.9821275495)
(1900,0.982272374)
(1910,0.9825067453)
(1920,0.9826698348)
(1930,0.9828001851)
(1940,0.9829720859)
(1950,0.9832251874)
(1960,0.9833668329)
(1970,0.9836212443)
(1980,0.9837293662)
(1990,0.9838870215)
(2000,0.9839568263)
(2010,0.9840349042)
(2020,0.9841365889)
(2030,0.9842555768)
(2040,0.9843911228)
(2050,0.9843815299)
(2060,0.9844200997)
(2070,0.9843770513)
(2080,0.9844306853)
(2090,0.9844453574)
(2100,0.9843856634)
(2110,0.9843672865)
(2120,0.9843488857)
(2130,0.9842250505)
(2140,0.9841666255)
(2150,0.9840919025)
(2160,0.9839516156)
(2170,0.9839094504)
(2180,0.9838593767)
(2190,0.9838260453)
(2200,0.9838085472)
(2210,0.9838494825)
(2220,0.9838409258)
(2230,0.9838646887)
(2240,0.9838232491)
(2250,0.9840269369)
(2260,0.9841497722)
(2270,0.9842893679)
(2280,0.9843134648)
(2290,0.9844782721)
(2300,0.9845278499)
(2310,0.9846523899)
(2320,0.9846276835)
(2330,0.9846944727)
(2340,0.9846371858)
(2350,0.9847036648)
(2360,0.9846963894)
(2370,0.9846392734)
(2380,0.984433198)
(2390,0.9843585502)
(2400,0.9842844843)
(2410,0.9842592128)
(2420,0.9839767726)
(2430,0.9839600844)
(2440,0.9838521906)
(2450,0.9837109532)
(2460,0.9835862185)
(2470,0.9834033596)
(2480,0.9833194888)
(2490,0.9832183213)
(2500,0.9829843701)};\label{plots:plot1}
\addplot[red] coordinates{(10,1)
(20,1)
};\label{plots:plot2}
\addplot[green] coordinates{(10,1)
(20,1)
};\label{plots:plot3}
\addplot[blue] coordinates{(0,1)
(10,1)
(20,1)
(30,1)
(40,1)
(50,1)
(60,1)
(70,1)
(80,1)
(90,1)
(100,1)
(110,1)
(120,1)
(130,1)
(140,1)
(150,1)
(160,1)
(170,1)
(180,1)
(190,1)
(200,1)
(210,1)
(220,1)
(230,1)
(240,1)
(250,1)
(260,1)
(270,1)
(280,1)
(290,1)
(300,1)
(310,0.9999989443)
(320,0.9999957771)
(330,0.9999757177)
(340,0.9998859679)
(350,0.9997517898)
(360,0.9997844119)
(370,0.9998413977)
(380,0.9997736336)
(390,0.999253879)
(400,0.9972579276)
(410,0.9935581175)
(420,0.9904120113)
(430,0.9891375664)
(440,0.9898793737)
(450,0.9914375398)
(460,0.9925890632)
(470,0.9933154477)
(480,0.9939224243)
(490,0.9948803178)
(500,0.9955965471)
(510,0.9961848881)
(520,0.9966193917)
(530,0.9969840882)
(540,0.9972761241)
(550,0.997525341)
(560,0.997723996)
(570,0.9978933257)
(580,0.9980324812)
(590,0.9981432476)
(600,0.9982352121)
(610,0.998311812)
(620,0.9983688514)
(630,0.9984072778)
(640,0.9984359087)
(650,0.9984519618)
(660,0.9984631275)
(670,0.9984627402)
(680,0.9984559435)
(690,0.9984426507)
(700,0.9984241216)
(710,0.9984109731)
(720,0.9984045952)
(730,0.99839564)
(740,0.9983867685)
(750,0.9983725749)
(760,0.9983584269)
(770,0.9983226038)
(780,0.9982894217)
(790,0.9982520756)
(800,0.9982160082)
(810,0.9981784939)
(820,0.9981408953)
(830,0.9981059691)
(840,0.99807097)
(850,0.9980428303)
(860,0.9980091009)
(870,0.9979780977)
(880,0.9979470478)
(890,0.9979075721)
(900,0.997876414)
(910,0.9978508226)
(920,0.9978209887)
(930,0.9977967568)
(940,0.997769685)
(950,0.9977468349)
(960,0.9977253914)
(970,0.9977067875)
(980,0.9976881875)
(990,0.9976724427)
(1000,0.9976567161)
(1010,0.9976481582)
(1020,0.9976396369)
(1030,0.9976340331)
(1040,0.99763279)
(1050,0.9976330473)
(1060,0.9976333671)
(1070,0.9976337496)
(1080,0.99763854)
(1090,0.9976463033)
(1100,0.9976570538)
(1110,0.9976693476)
(1120,0.9976831914)
(1130,0.997697126)
(1140,0.9977170053)
(1150,0.9977355258)
(1160,0.9977526836)
(1170,0.9977699389)
(1180,0.9977917107)
(1190,0.9978121164)
(1200,0.9978311455)
(1210,0.9978487942)
(1220,0.9978680123)
(1230,0.9978843577)
(1240,0.9979022714)
(1250,0.9979187835)
(1260,0.9979249713)
(1270,0.9979327009)
(1280,0.99793452)
(1290,0.9979363776)
(1300,0.9979397712)
(1310,0.9979417082)
(1320,0.997942183)
(1330,0.9979441896)
(1340,0.9979477365)
(1350,0.9979498134)
(1360,0.997950421)
(1370,0.9979540777)
(1380,0.9979547506)
(1390,0.997956963)
(1400,0.9979561814)
(1410,0.9979569395)
(1420,0.9979562057)
(1430,0.9979554983)
(1440,0.9979517739)
(1450,0.997958708)
(1460,0.9979641539)
(1470,0.9979681126)
(1480,0.9979690482)
(1490,0.9979715404)
(1500,0.997971003)
(1510,0.9979735457)
(1520,0.9979822468)
(1530,0.9979925169)
(1540,0.9980043603)
(1550,0.9980224015)
(1560,0.9980389559)
(1570,0.9980571027)
(1580,0.9980768459)
(1590,0.9980966447)
(1600,0.9981164987)
(1610,0.9981348597)
(1620,0.9981532722)
(1630,0.998171733)
(1640,0.9981902475)
(1650,0.9982072589)
(1660,0.9982227626)
(1670,0.9982351952)
(1680,0.9982461114)
(1690,0.9982586165)
(1700,0.9982680389)
(1710,0.9982790527)
(1720,0.9982869727)
(1730,0.9982949195)
(1740,0.9982981988)
(1750,0.9983014915)
(1760,0.998301672)
(1770,0.9983018634)
(1780,0.9983004951)
(1790,0.9982912889)
(1800,0.9982820762)
(1810,0.9982712881)
(1820,0.9982620671)
(1830,0.9982544223)
(1840,0.9982483521)
(1850,0.9982422865)
(1860,0.9982409642)
(1870,0.9982443904)
(1880,0.9982494155)
(1890,0.9982592085)
(1900,0.998270612)
(1910,0.9982788733)
(1920,0.9982887422)
(1930,0.9982954564)
(1940,0.9983037806)
(1950,0.998310534)
(1960,0.9983157157)
(1970,0.9983193197)
(1980,0.9983245282)
(1990,0.9983281593)
(2000,0.9983302071)
(2010,0.9983322657)
(2020,0.9983343377)
(2030,0.9983348183)
(2040,0.9983369082)
(2050,0.998335808)
(2060,0.9983363172)
(2070,0.9983384362)
(2080,0.9983389637)
(2090,0.9983394973)
(2100,0.9983384327)
(2110,0.9983405879)
(2120,0.9983411449)
(2130,0.9983401007)
(2140,0.9983406714)
(2150,0.9983428603)
(2160,0.9983418365)
(2170,0.9983424309)
(2180,0.9983414163)
(2190,0.9983436378)
(2200,0.9983442531)
(2210,0.9983432565)
(2220,0.998340648)
(2230,0.9983412814)
(2240,0.9983419209)
(2250,0.9983425665)
(2260,0.9983432156)
(2270,0.9983487391)
(2280,0.998351028)
(2290,0.9983549503)
(2300,0.9983588799)
(2310,0.9983628221)
(2320,0.99836352)
(2330,0.9983674799)
(2340,0.998368192)
(2350,0.9983721723)
(2360,0.9983761597)
(2370,0.9983785267)
(2380,0.9983825353)
(2390,0.9983849189)
(2400,0.998388946)
(2410,0.9983929828)
(2420,0.9983953918)
(2430,0.9983978087)
(2440,0.9984002334)
(2450,0.9984026659)
(2460,0.9984067471)
(2470,0.9984075544)
(2480,0.9984083678)
(2490,0.9984108281)
(2500,0.9984149403)};\label{plots:plot4}

==> charts/exponential_decay_approx.tex <==
\addplot[black] coordinates{(0,1.0000)
(15,1.0000)
(30,1.0000)
(45,1.0000)
(60,1.0000)
(75,1.0000)
(90,1.0000)
(105,1.0052)
(120,1.0253)
(135,1.0343)
(150,1.0348)
(165,1.0294)
(180,1.0160)
(195,0.9959)
(210,0.9640)
(225,0.9322)
(240,0.9013)
(255,0.8865)
(270,0.9039)
(285,0.9077)
(300,0.9069)
(315,0.9075)
(330,0.9094)
(345,0.9118)
(360,0.9147)
(375,0.9176)
(390,0.9207)
(405,0.9240)
(420,0.9271)
(435,0.9301)
(450,0.9330)
(465,0.9359)
(480,0.9386)
(495,0.9412)
(510,0.9436)
(525,0.9461)
(540,0.9484)
(555,0.9507)
(570,0.9528)
(585,0.9547)
(600,0.9566)
(615,0.9584)
(630,0.9600)
(645,0.9617)
(660,0.9633)
(675,0.9649)
(690,0.9665)
(705,0.9681)
(720,0.9697)
(735,0.9711)
(750,0.9725)
(765,0.9739)
(780,0.9752)
(795,0.9763)
(810,0.9774)
(825,0.9785)
(840,0.9795)
(855,0.9804)
(870,0.9814)
(885,0.9824)
(900,0.9832)
(915,0.9841)
(930,0.9849)
(945,0.9858)
(960,0.9867)
(975,0.9877)
(990,0.9886)
(1005,0.9895)
(1020,0.9904)
(1035,0.9914)
(1050,0.9925)
(1065,0.9937)
(1080,0.9948)
(1095,0.9959)
(1110,0.9970)
(1125,0.9982)
(1140,0.9997)
(1155,1.0011)
(1170,1.0026)
(1185,1.0041)
(1200,1.0057)
(1215,1.0072)
(1230,1.0088)
(1245,1.0106)
(1260,1.0124)
(1275,1.0143)
(1290,1.0161)
(1305,1.0177)
(1320,1.0194)
(1335,1.0210)
(1350,1.0225)
(1365,1.0241)
(1380,1.0256)
(1395,1.0272)
(1410,1.0285)
(1425,1.0298)
(1440,1.0309)
(1455,1.0320)
(1470,1.0331)
(1485,1.0339)
(1500,1.0347)
(1515,1.0356)
(1530,1.0362)
(1545,1.0368)
(1560,1.0376)
(1575,1.0383)
(1590,1.0389)
(1605,1.0394)
(1620,1.0399)
(1635,1.0403)
(1650,1.0404)
(1665,1.0407)
(1680,1.0409)
(1695,1.0410)
(1710,1.0411)
(1725,1.0412)
(1740,1.0413)
(1755,1.0412)
(1770,1.0411)
(1785,1.0412)
(1800,1.0411)
(1815,1.0412)
(1830,1.0411)
(1845,1.0409)
(1860,1.0408)
(1875,1.0406)
(1890,1.0405)
(1905,1.0402)
(1920,1.0400)
(1935,1.0397)
(1950,1.0396)
(1965,1.0395)
(1980,1.0393)
(1995,1.0391)
(2010,1.0389)
(2025,1.0386)
(2040,1.0384)
(2055,1.0382)
(2070,1.0379)
(2085,1.0378)
(2100,1.0376)
(2115,1.0374)
(2130,1.0371)
(2145,1.0368)
(2160,1.0365)
(2175,1.0362)
(2190,1.0358)
(2205,1.0356)
(2220,1.0353)
(2235,1.0349)
(2250,1.0346)
(2265,1.0342)
(2280,1.0338)
(2295,1.0334)
(2310,1.0330)
(2325,1.0327)
(2340,1.0323)
(2355,1.0319)
(2370,1.0315)
(2385,1.0312)
(2400,1.0309)
(2415,1.0306)
(2430,1.0303)
(2445,1.0301)
(2460,1.0298)
(2475,1.0295)
(2490,1.0293)
(2500,1.0290)};\label{plots:plot1}
\addplot[red] coordinates{(0,1.0000)
(10,1.0000)
(20,1.0000)
(30,1.0000)
(40,1.0000)
(50,1.0000)
(60,1.0000)
(70,1.0000)
(80,1.0000)
(90,1.0000)
(100,1.0000)
(110,1.0000)
(120,1.0000)
(130,1.0000)
(140,1.0000)
(150,1.0000)
(160,1.0000)
(170,0.9980)
(180,0.9810)
(190,0.9513)
(200,0.9250)
(210,0.9022)
(220,0.8832)
(230,0.8670)
(240,0.8526)
(250,0.8411)
(260,0.8729)
(270,0.9024)
(280,0.9206)
(290,0.9319)
(300,0.9399)
(310,0.9459)
(320,0.9507)
(330,0.9546)
(340,0.9579)
(350,0.9607)
(360,0.9633)
(370,0.9655)
(380,0.9675)
(390,0.9692)
(400,0.9708)
(410,0.9723)
(420,0.9736)
(430,0.9748)
(440,0.9759)
(450,0.9770)
(460,0.9781)
(470,0.9790)
(480,0.9798)
(490,0.9805)
(500,0.9813)
(510,0.9820)
(520,0.9826)
(530,0.9832)
(540,0.9838)
(550,0.9844)
(560,0.9850)
(570,0.9855)
(580,0.9860)
(590,0.9865)
(600,0.9869)
(610,0.9874)
(620,0.9878)
(630,0.9882)
(640,0.9886)
(650,0.9890)
(660,0.9894)
(670,0.9897)
(680,0.9900)
(690,0.9904)
(700,0.9907)
(710,0.9911)
(720,0.9915)
(730,0.9918)
(740,0.9922)
(750,0.9925)
(760,0.9928)
(770,0.9930)
(780,0.9933)
(790,0.9936)
(800,0.9939)
(810,0.9941)
(820,0.9944)
(830,0.9946)
(840,0.9948)
(850,0.9950)
(860,0.9952)
(870,0.9954)
(880,0.9956)
(890,0.9957)
(900,0.9959)
(910,0.9961)
(920,0.9962)
(930,0.9964)
(940,0.9965)
(950,0.9966)
(960,0.9968)
(970,0.9969)
(980,0.9970)
(990,0.9971)
(1000,0.9972)
(1010,0.9973)
(1020,0.9974)
(1030,0.9975)
(1040,0.9976)
(1050,0.9977)
(1060,0.9978)
(1070,0.9978)
(1080,0.9979)
(1090,0.9980)
(1100,0.9981)
(1110,0.9981)
(1120,0.9982)
(1130,0.9983)
(1140,0.9984)
(1150,0.9985)
(1160,0.9986)
(1170,0.9987)
(1180,0.9988)
(1190,0.9989)
(1200,0.9990)
(1210,0.9991)
(1220,0.9992)
(1230,0.9992)
(1240,0.9993)
(1250,0.9994)
(1260,0.9995)
(1270,0.9996)
(1280,0.9996)
(1290,0.9997)
(1300,0.9998)
(1310,0.9998)
(1320,0.9999)
(1330,1.0000)
(1340,1.0000)
(1350,1.0001)
(1360,1.0002)
(1370,1.0003)
(1380,1.0003)
(1390,1.0004)
(1400,1.0005)
(1410,1.0005)
(1420,1.0006)
(1430,1.0007)
(1440,1.0007)
(1450,1.0008)
(1460,1.0009)
(1470,1.0009)
(1480,1.0010)
(1490,1.0011)
(1500,1.0012)
(1510,1.0013)
(1520,1.0013)
(1530,1.0014)
(1540,1.0014)
(1550,1.0015)
(1560,1.0016)
(1570,1.0016)
(1580,1.0017)
(1590,1.0018)
(1600,1.0018)
(1610,1.0019)
(1620,1.0019)
(1630,1.0020)
(1640,1.0021)
(1650,1.0021)
(1660,1.0022)
(1670,1.0022)
(1680,1.0023)
(1690,1.0023)
(1700,1.0024)
(1710,1.0024)
(1720,1.0025)
(1730,1.0025)
(1740,1.0026)
(1750,1.0027)
(1760,1.0027)
(1770,1.0028)
(1780,1.0028)
(1790,1.0029)
(1800,1.0029)
(1810,1.0030)
(1820,1.0031)
(1830,1.0031)
(1840,1.0032)
(1850,1.0032)
(1860,1.0033)
(1870,1.0033)
(1880,1.0034)
(1890,1.0034)
(1900,1.0035)
(1910,1.0035)
(1920,1.0036)
(1930,1.0036)
(1940,1.0037)
(1950,1.0038)
(1960,1.0038)
(1970,1.0039)
(1980,1.0039)
(1990,1.0040)
(2000,1.0040)
(2010,1.0041)
(2020,1.0042)
(2030,1.0042)
(2040,1.0043)
(2050,1.0043)
(2060,1.0043)
(2070,1.0044)
(2080,1.0045)
(2090,1.0045)
(2100,1.0045)
(2110,1.0046)
(2120,1.0046)
(2130,1.0047)
(2140,1.0047)
(2150,1.0048)
(2160,1.0048)
(2170,1.0049)
(2180,1.0049)
(2190,1.0050)
(2200,1.0051)
(2210,1.0051)
(2220,1.0052)
(2230,1.0053)
(2240,1.0053)
(2250,1.0053)
(2260,1.0054)
(2270,1.0054)
(2280,1.0055)
(2290,1.0056)
(2300,1.0057)
(2310,1.0057)
(2320,1.0058)
(2330,1.0059)
(2340,1.0060)
(2350,1.0061)
(2360,1.0062)
(2370,1.0063)
(2380,1.0065)
(2390,1.0066)
(2400,1.0067)
(2410,1.0068)
(2420,1.0069)
(2430,1.0070)
(2440,1.0072)
(2450,1.0073)
(2460,1.0074)
(2470,1.0076)
(2480,1.0077)
(2490,1.0078)
(2500,1.0080)
};\label{plots:plot2}
\addplot[green] coordinates{(0,1)
(10,1)
(20,1)
(30,1)
(40,1)
(50,1)
(60,1)
(70,1)
(80,1)
(90,1)
(100,1)
(110,1)
(120,1)
(130,1)
(140,1)
(150,1)
(160,1)
(170,1)
(180,1)
(190,0.9999985588)
(200,0.9998184064)
(210,0.9935324724)
(220,0.9589196688)
(230,0.9349902669)
(240,0.9189209517)
(250,0.8998312381)
(260,0.9044424681)
(270,0.9092646426)
(280,0.9147082913)
(290,0.9234508131)
(300,0.9322543712)
(310,0.9397240166)
(320,0.9456482107)
(330,0.9504229464)
(340,0.9545936255)
(350,0.9582974165)
(360,0.9616176499)
(370,0.9646725363)
(380,0.9674790494)
(390,0.970043363)
(400,0.9724191347)
(410,0.9746423089)
(420,0.9767074167)
(430,0.9786117516)
(440,0.980361451)
(450,0.9819615664)
(460,0.98346081)
(470,0.9849140172)
(480,0.9863021995)
(490,0.9876169885)
(500,0.9889150427)
(510,0.990184993)
(520,0.9913837173)
(530,0.9924756656)
(540,0.9934867193)
(550,0.9944431591)
(560,0.9953482276)
(570,0.9962268461)
(580,0.9970612386)
(590,0.9978636784)
(600,0.9986206207)
(610,0.999383696)
(620,1.00010042)
(630,1.000794307)
(640,1.00144747)
(650,1.002079276)
(660,1.002693856)
(670,1.003271112)
(680,1.003819546)
(690,1.004336621)
(700,1.0048132)
(710,1.005262362)
(720,1.005697352)
(730,1.006106788)
(740,1.006524053)
(750,1.006973729)
(760,1.007406577)
(770,1.007824716)
(780,1.008228092)
(790,1.00862337)
(800,1.009001467)
(810,1.009375805)
(820,1.009737255)
(830,1.010078923)
(840,1.010421299)
(850,1.010750587)
(860,1.011057579)
(870,1.01138121)
(880,1.011698494)
(890,1.012011799)
(900,1.012316358)
(910,1.012607619)
(920,1.012910809)
(930,1.013195983)
(940,1.013488564)
(950,1.013779152)
(960,1.014065481)
(970,1.014345183)
(980,1.01461374)
(990,1.014870935)
(1000,1.015126132)
(1010,1.015381591)
(1020,1.015639615)
(1030,1.015886295)
(1040,1.016114441)
(1050,1.016335893)
(1060,1.016564533)
(1070,1.016776955)
(1080,1.01698494)
(1090,1.017190722)
(1100,1.017384755)
(1110,1.017579073)
(1120,1.017771051)
(1130,1.017958375)
(1140,1.018145789)
(1150,1.018326305)
(1160,1.018497429)
(1170,1.018687666)
(1180,1.018859069)
(1190,1.019023418)
(1200,1.019192487)
(1210,1.019363974)
(1220,1.019516512)
(1230,1.019669173)
(1240,1.019814698)
(1250,1.019972122)
(1260,1.020117771)
(1270,1.02026352)
(1280,1.020402183)
(1290,1.020543151)
(1300,1.020679325)
(1310,1.020820409)
(1320,1.020949529)
(1330,1.021095356)
(1340,1.021233996)
(1350,1.021370281)
(1360,1.021501826)
(1370,1.021635752)
(1380,1.021767252)
(1390,1.021908474)
(1400,1.022044837)
(1410,1.022171618)
(1420,1.022303309)
(1430,1.022437373)
(1440,1.022568985)
(1450,1.02270047)
(1460,1.022824768)
(1470,1.022965926)
(1480,1.023104678)
(1490,1.023233672)
(1500,1.023372483)
(1510,1.023506423)
(1520,1.023628292)
(1530,1.023764721)
(1540,1.023893863)
(1550,1.024001075)
(1560,1.024127766)
(1570,1.02424468)
(1580,1.024361528)
(1590,1.024478424)
(1600,1.024590381)
(1610,1.024702497)
(1620,1.024817002)
(1630,1.024924144)
(1640,1.025048365)
(1650,1.02516028)
(1660,1.025252757)
(1670,1.025357494)
(1680,1.025462075)
(1690,1.025554362)
(1700,1.02565403)
(1710,1.025753593)
(1720,1.025845858)
(1730,1.02594055)
(1740,1.026030227)
(1750,1.026127231)
(1760,1.026234183)
(1770,1.026338732)
(1780,1.026433287)
(1790,1.026525488)
(1800,1.026612586)
(1810,1.026702302)
(1820,1.026772219)
(1830,1.026851892)
(1840,1.026926635)
(1850,1.027001428)
(1860,1.02707358)
(1870,1.027145714)
(1880,1.027212703)
(1890,1.027279669)
(1900,1.027339446)
(1910,1.027403994)
(1920,1.027476018)
(1930,1.027545385)
(1940,1.027609723)
(1950,1.027669159)
(1960,1.027723486)
(1970,1.027777913)
(1980,1.027839619)
(1990,1.027898786)
(2000,1.027945514)
(2010,1.027999658)
(2020,1.028053764)
(2030,1.028092974)
(2040,1.028139601)
(2050,1.028178718)
(2060,1.028215204)
(2070,1.028259042)
(2080,1.028287955)
(2090,1.028324289)
(2100,1.028343032)
(2110,1.028374087)
(2120,1.028390194)
(2130,1.028413861)
(2140,1.028432294)
(2150,1.028440731)
(2160,1.028454)
(2170,1.028452227)
(2180,1.028460325)
(2190,1.028453372)
(2200,1.02845384)
(2210,1.028444152)
(2220,1.028429558)
(2230,1.028424837)
(2240,1.028400143)
(2250,1.028390231)
(2260,1.028380524)
(2270,1.028365626)
(2280,1.028348061)
(2290,1.02832551)
(2300,1.028302813)
(2310,1.028257245)
(2320,1.028219102)
(2330,1.028183475)
(2340,1.028132615)
(2350,1.028079149)
(2360,1.028028129)
(2370,1.027977029)
(2380,1.027928238)
(2390,1.027879369)
(2400,1.027823116)
(2410,1.027764052)
(2420,1.027712558)
(2430,1.027660919)
(2440,1.027606811)
(2450,1.027552559)
(2460,1.027490581)
(2470,1.027430986)
(2480,1.027379031)
(2490,1.027319286)
(2500,1.027242044)};\label{plots:plot3}
\addplot[blue] coordinates{(0,1.000)
(10,1.000)};\label{plots:plot4}
\addplot[dashed,black] coordinates{(0,1.000)
(10,1.000)
(20,1.000)
(30,1.000)
(40,1.000)
(50,1.000)
(60,1.000)
(70,1.000)
(80,1.000)
(90,1.000)
(100,1.002)
(110,1.020)
(120,1.027)
(130,1.033)
(140,1.033)
(150,1.033)
(160,1.035)
(170,1.039)
(180,1.044)
(190,1.049)
(200,1.053)
(210,1.057)
(220,1.060)
(230,1.063)
(240,1.065)
(250,1.066)
(260,1.049)
(270,1.043)
(280,1.044)
(290,1.042)
(300,1.039)
(310,1.037)
(320,1.035)
(330,1.034)
(340,1.033)
(350,1.033)
(360,1.032)
(370,1.032)
(380,1.031)
(390,1.031)
(400,1.031)
(410,1.031)
(420,1.031)
(430,1.031)
(440,1.031)
(450,1.032)
(460,1.032)
(470,1.032)
(480,1.032)
(490,1.032)
(500,1.032)
(510,1.032)
(520,1.032)
(530,1.032)
(540,1.032)
(550,1.032)
(560,1.032)
(570,1.033)
(580,1.033)
(590,1.033)
(600,1.033)
(610,1.033)
(620,1.033)
(630,1.033)
(640,1.033)
(650,1.033)
(660,1.033)
(670,1.033)
(680,1.033)
(690,1.034)
(700,1.034)
(710,1.034)
(720,1.034)
(730,1.034)
(740,1.034)
(750,1.034)
(760,1.035)
(770,1.035)
(780,1.035)
(790,1.035)
(800,1.035)
(810,1.035)
(820,1.035)
(830,1.035)
(840,1.035)
(850,1.035)
(860,1.035)
(870,1.036)
(880,1.036)
(890,1.036)
(900,1.036)
(910,1.036)
(920,1.036)
(930,1.036)
(940,1.037)
(950,1.037)
(960,1.037)
(970,1.037)
(980,1.037)
(990,1.038)
(1000,1.038)
(1010,1.038)
(1020,1.038)
(1030,1.039)
(1040,1.039)
(1050,1.039)
(1060,1.039)
(1070,1.039)
(1080,1.040)
(1090,1.040)
(1100,1.040)
(1110,1.041)
(1120,1.041)
(1130,1.041)
(1140,1.041)
(1150,1.042)
(1160,1.042)
(1170,1.042)
(1180,1.042)
(1190,1.043)
(1200,1.043)
(1210,1.043)
(1220,1.044)
(1230,1.044)
(1240,1.044)
(1250,1.044)
(1260,1.044)
(1270,1.044)
(1280,1.045)
(1290,1.045)
(1300,1.045)
(1310,1.046)
(1320,1.046)
(1330,1.046)
(1340,1.046)
(1350,1.046)
(1360,1.047)
(1370,1.047)
(1380,1.047)
(1390,1.047)
(1400,1.047)
(1410,1.047)
(1420,1.047)
(1430,1.047)
(1440,1.047)
(1450,1.047)
(1460,1.047)
(1470,1.047)
(1480,1.047)
(1490,1.047)
(1500,1.048)
(1510,1.047)
(1520,1.047)
(1530,1.047)
(1540,1.047)
(1550,1.047)
(1560,1.047)
(1570,1.047)
(1580,1.047)
(1590,1.047)
(1600,1.047)
(1610,1.047)
(1620,1.047)
(1630,1.047)
(1640,1.047)
(1650,1.047)
(1660,1.047)
(1670,1.047)
(1680,1.047)
(1690,1.047)
(1700,1.046)
(1710,1.046)
(1720,1.046)
(1730,1.046)
(1740,1.046)
(1750,1.046)
(1760,1.046)
(1770,1.046)
(1780,1.046)
(1790,1.046)
(1800,1.046)
(1810,1.045)
(1820,1.045)
(1830,1.045)
(1840,1.045)
(1850,1.045)
(1860,1.045)
(1870,1.045)
(1880,1.045)
(1890,1.045)
(1900,1.045)
(1910,1.045)
(1920,1.044)
(1930,1.044)
(1940,1.044)
(1950,1.044)
(1960,1.044)
(1970,1.044)
(1980,1.044)
(1990,1.044)
(2000,1.044)
(2010,1.044)
(2020,1.044)
(2030,1.044)
(2040,1.044)
(2050,1.044)
(2060,1.044)
(2070,1.044)
(2080,1.044)
(2090,1.044)
(2100,1.044)
(2110,1.044)
(2120,1.044)
(2130,1.044)
(2140,1.044)
(2150,1.044)
(2160,1.045)
(2170,1.045)
(2180,1.045)
(2190,1.045)
(2200,1.045)
(2210,1.045)
(2220,1.045)
(2230,1.045)
(2240,1.045)
(2250,1.045)
(2260,1.045)
(2270,1.046)
(2280,1.046)
(2290,1.046)
(2300,1.046)
(2310,1.046)
(2320,1.046)
(2330,1.046)
(2340,1.046)
(2350,1.046)
(2360,1.046)
(2370,1.046)
(2380,1.047)
(2390,1.047)
(2400,1.047)
(2410,1.047)
(2420,1.047)
(2430,1.047)
(2440,1.047)
(2450,1.047)
(2460,1.048)
(2470,1.048)
(2480,1.048)
(2490,1.048)
(2500,1.048)
};\label{plots:plot5}
\addplot[dashed,red] coordinates{(0,1.000)
(10,1.000)
(20,1.000)
(30,1.000)
(40,1.000)
(50,1.000)
(60,1.000)
(70,1.000)
(80,1.000)
(90,1.000)
(100,1.000)
(110,1.004)
(120,1.008)
(130,1.007)
(140,1.008)
(150,1.009)
(160,1.009)
(170,1.009)
(180,1.009)
(190,1.010)
(200,1.010)
(210,1.010)
(220,1.010)
(230,1.010)
(240,1.010)
(250,1.010)
(260,1.005)
(270,1.003)
(280,1.001)
(290,1.001)
(300,1.001)
(310,1.001)
(320,1.001)
(330,1.001)
(340,1.001)
(350,1.001)
(360,1.001)
(370,1.001)
(380,1.001)
(390,1.001)
(400,1.001)
(410,1.001)
(420,1.001)
(430,1.001)
(440,1.001)
(450,1.001)
(460,1.001)
(470,1.002)
(480,1.002)
(490,1.002)
(500,1.002)
(510,1.002)
(520,1.002)
(530,1.002)
(540,1.002)
(550,1.002)
(560,1.002)
(570,1.002)
(580,1.002)
(590,1.002)
(600,1.002)
(610,1.002)
(620,1.002)
(630,1.002)
(640,1.003)
(650,1.003)
(660,1.003)
(670,1.003)
(680,1.003)
(690,1.003)
(700,1.003)
(710,1.003)
(720,1.003)
(730,1.003)
(740,1.003)
(750,1.003)
(760,1.003)
(770,1.003)
(780,1.003)
(790,1.003)
(800,1.003)
(810,1.003)
(820,1.003)
(830,1.004)
(840,1.004)
(850,1.004)
(860,1.004)
(870,1.004)
(880,1.004)
(890,1.004)
(900,1.004)
(910,1.004)
(920,1.004)
(930,1.004)
(940,1.004)
(950,1.004)
(960,1.004)
(970,1.004)
(980,1.004)
(990,1.004)
(1000,1.004)
(1010,1.004)
(1020,1.004)
(1030,1.004)
(1040,1.004)
(1050,1.004)
(1060,1.004)
(1070,1.004)
(1080,1.004)
(1090,1.004)
(1100,1.004)
(1110,1.004)
(1120,1.004)
(1130,1.004)
(1140,1.004)
(1150,1.004)
(1160,1.004)
(1170,1.004)
(1180,1.004)
(1190,1.004)
(1200,1.004)
(1210,1.004)
(1220,1.004)
(1230,1.004)
(1240,1.004)
(1250,1.004)
(1260,1.004)
(1270,1.005)
(1280,1.005)
(1290,1.005)
(1300,1.005)
(1310,1.005)
(1320,1.005)
(1330,1.005)
(1340,1.005)
(1350,1.005)
(1360,1.005)
(1370,1.005)
(1380,1.005)
(1390,1.005)
(1400,1.005)
(1410,1.005)
(1420,1.005)
(1430,1.005)
(1440,1.005)
(1450,1.005)
(1460,1.005)
(1470,1.005)
(1480,1.005)
(1490,1.005)
(1500,1.005)
(1510,1.005)
(1520,1.005)
(1530,1.005)
(1540,1.005)
(1550,1.005)
(1560,1.005)
(1570,1.005)
(1580,1.005)
(1590,1.005)
(1600,1.005)
(1610,1.005)
(1620,1.005)
(1630,1.005)
(1640,1.005)
(1650,1.005)
(1660,1.005)
(1670,1.005)
(1680,1.005)
(1690,1.005)
(1700,1.005)
(1710,1.005)
(1720,1.005)
(1730,1.005)
(1740,1.005)
(1750,1.005)
(1760,1.005)
(1770,1.005)
(1780,1.005)
(1790,1.005)
(1800,1.005)
(1810,1.005)
(1820,1.005)
(1830,1.005)
(1840,1.005)
(1850,1.005)
(1860,1.005)
(1870,1.005)
(1880,1.005)
(1890,1.005)
(1900,1.005)
(1910,1.005)
(1920,1.005)
(1930,1.005)
(1940,1.005)
(1950,1.005)
(1960,1.005)
(1970,1.005)
(1980,1.005)
(1990,1.005)
(2000,1.005)
(2010,1.005)
(2020,1.005)
(2030,1.005)
(2040,1.006)
(2050,1.006)
(2060,1.006)
(2070,1.006)
(2080,1.006)
(2090,1.006)
(2100,1.006)
(2110,1.006)
(2120,1.006)
(2130,1.006)
(2140,1.006)
(2150,1.006)
(2160,1.006)
(2170,1.006)
(2180,1.006)
(2190,1.007)
(2200,1.007)
(2210,1.007)
(2220,1.007)
(2230,1.007)
(2240,1.007)
(2250,1.007)
(2260,1.007)
(2270,1.007)
(2280,1.007)
(2290,1.007)
(2300,1.007)
(2310,1.007)
(2320,1.007)
(2330,1.007)
(2340,1.007)
(2350,1.007)
(2360,1.007)
(2370,1.007)
(2380,1.007)
(2390,1.007)
(2400,1.007)
(2410,1.007)
(2420,1.007)
(2430,1.007)
(2440,1.007)
(2450,1.007)
(2460,1.008)
(2470,1.008)
(2480,1.008)
(2490,1.008)
(2500,1.008)};\label{plots:plot6}
\addplot[dashed,green] coordinates{
(0,1.000)
(10,1.000)
(20,1.000)
(30,1.000)
(40,1.000)
(50,1.000)
(60,1.000)
(70,1.000)
(80,1.000)
(90,1.000)
(100,1.000)
(110,1.000)
(120,1.000)
(130,1.000)
(140,1.000)
(150,1.000)
(160,1.000)
(170,1.000)
(180,1.000)
(190,1.000)
(200,1.000)
(210,1.000)
(220,1.002)
(230,1.007)
(240,1.009)
(250,1.006)
(260,1.002)
(270,1.002)
(280,1.003)
(290,1.003)
(300,1.001)
(310,1.000)
(320,0.999)
(330,0.999)
(340,0.999)
(350,1.000)
(360,1.000)
(370,1.000)
(380,1.001)
(390,1.002)
(400,1.002)
(410,1.003)
(420,1.003)
(430,1.004)
(440,1.004)
(450,1.005)
(460,1.005)
(470,1.006)
(480,1.006)
(490,1.006)
(500,1.007)
(510,1.007)
(520,1.008)
(530,1.008)
(540,1.008)
(550,1.009)
(560,1.009)
(570,1.009)
(580,1.010)
(590,1.010)
(600,1.011)
(610,1.011)
(620,1.011)
(630,1.012)
(640,1.012)
(650,1.012)
(660,1.013)
(670,1.013)
(680,1.013)
(690,1.013)
(700,1.014)
(710,1.014)
(720,1.014)
(730,1.014)
(740,1.015)
(750,1.015)
(760,1.015)
(770,1.015)
(780,1.015)
(790,1.016)
(800,1.016)
(810,1.016)
(820,1.016)
(830,1.016)
(840,1.017)
(850,1.017)
(860,1.017)
(870,1.017)
(880,1.017)
(890,1.017)
(900,1.018)
(910,1.018)
(920,1.018)
(930,1.018)
(940,1.018)
(950,1.018)
(960,1.019)
(970,1.019)
(980,1.019)
(990,1.019)
(1000,1.019)
(1010,1.019)
(1020,1.020)
(1030,1.020)
(1040,1.020)
(1050,1.020)
(1060,1.020)
(1070,1.020)
(1080,1.021)
(1090,1.021)
(1100,1.021)
(1110,1.021)
(1120,1.021)
(1130,1.021)
(1140,1.021)
(1150,1.022)
(1160,1.022)
(1170,1.022)
(1180,1.022)
(1190,1.022)
(1200,1.022)
(1210,1.022)
(1220,1.023)
(1230,1.023)
(1240,1.023)
(1250,1.023)
(1260,1.023)
(1270,1.023)
(1280,1.023)
(1290,1.023)
(1300,1.023)
(1310,1.024)
(1320,1.024)
(1330,1.024)
(1340,1.024)
(1350,1.024)
(1360,1.024)
(1370,1.024)
(1380,1.024)
(1390,1.024)
(1400,1.025)
(1410,1.025)
(1420,1.025)
(1430,1.025)
(1440,1.025)
(1450,1.025)
(1460,1.025)
(1470,1.025)
(1480,1.025)
(1490,1.026)
(1500,1.026)
(1510,1.026)
(1520,1.026)
(1530,1.026)
(1540,1.026)
(1550,1.026)
(1560,1.026)
(1570,1.026)
(1580,1.026)
(1590,1.027)
(1600,1.027)
(1610,1.027)
(1620,1.027)
(1630,1.027)
(1640,1.027)
(1650,1.027)
(1660,1.027)
(1670,1.027)
(1680,1.027)
(1690,1.027)
(1700,1.028)
(1710,1.028)
(1720,1.028)
(1730,1.028)
(1740,1.028)
(1750,1.028)
(1760,1.028)
(1770,1.028)
(1780,1.028)
(1790,1.028)
(1800,1.028)
(1810,1.028)
(1820,1.029)
(1830,1.029)
(1840,1.029)
(1850,1.029)
(1860,1.029)
(1870,1.029)
(1880,1.029)
(1890,1.029)
(1900,1.029)
(1910,1.029)
(1920,1.029)
(1930,1.029)
(1940,1.029)
(1950,1.030)
(1960,1.030)
(1970,1.030)
(1980,1.030)
(1990,1.030)
(2000,1.030)
(2010,1.030)
(2020,1.030)
(2030,1.030)
(2040,1.030)
(2050,1.030)
(2060,1.030)
(2070,1.030)
(2080,1.031)
(2090,1.031)
(2100,1.031)
(2110,1.031)
(2120,1.031)
(2130,1.031)
(2140,1.031)
(2150,1.031)
(2160,1.031)
(2170,1.031)
(2180,1.031)
(2190,1.031)
(2200,1.031)
(2210,1.031)
(2220,1.031)
(2230,1.031)
(2240,1.031)
(2250,1.031)
(2260,1.031)
(2270,1.031)
(2280,1.031)
(2290,1.031)
(2300,1.031)
(2310,1.031)
(2320,1.031)
(2330,1.031)
(2340,1.031)
(2350,1.031)
(2360,1.031)
(2370,1.031)
(2380,1.031)
(2390,1.031)
(2400,1.031)
(2410,1.031)
(2420,1.031)
(2430,1.031)
(2440,1.031)
(2450,1.031)
(2460,1.031)
(2470,1.031)
(2480,1.031)
(2490,1.031)
(2500,1.031)};\label{plots:plot7}
\addplot[dashed,blue] coordinates{(0,1)
(10,1)
(20,1)
(30,1)
(40,1)
(50,1)
(60,1)
(70,1)
(80,1)
(90,1)
(100,1)
(110,1)
(120,1)
(130,1.000004169)
(140,1.000008349)
(150,1.000008355)
(160,1.000005572)
(170,1.00000418)
(180,1)
(190,0.9999818838)
(200,0.9998996492)
(210,0.9995245041)
(220,0.9981918485)
(230,0.9969353425)
(240,0.9986715165)
(250,1.000366636)
(260,1.000065519)
(270,0.998460039)
(280,0.9853170781)
(290,0.9794679619)
(300,0.9851605687)
(310,0.988468002)
(320,0.9899835506)
(330,0.9907058562)
(340,0.9910107847)
(350,0.9910535286)
(360,0.99092083)
(370,0.9907119238)
(380,0.9904895586)
(390,0.9902463917)
(400,0.9899748799)
(410,0.989702902)
(420,0.9894279345)
(430,0.9891941634)
(440,0.9890217887)
(450,0.9888576613)
(460,0.9886954058)
(470,0.9885740603)
(480,0.9884549538)
(490,0.9883663136)
(500,0.9882995007)
(510,0.9882615786)
(520,0.9882147101)
(530,0.9881989055)
(540,0.9881830601)
(550,0.9881894627)
(560,0.9882160182)
(570,0.9882540034)
(580,0.9882732547)
(590,0.9882874873)
(600,0.9883033692)
(610,0.9883348544)
(620,0.9883656301)
(630,0.9884071949)
(640,0.9884408972)
(650,0.9884713462)
(660,0.9884888305)
(670,0.9884979491)
(680,0.9884962095)
(690,0.9884953745)
(700,0.9884906122)
(710,0.9884866864)
(720,0.9884908275)
(730,0.9885055506)
(740,0.9885090132)
(750,0.9885205711)
(760,0.9885426982)
(770,0.9885705675)
(780,0.9886041368)
(790,0.9886385648)
(800,0.9886614032)
(810,0.9886824573)
(820,0.9886991795)
(830,0.9887365353)
(840,0.9887796132)
(850,0.9888384192)
(860,0.9889029819)
(870,0.9889707465)
(880,0.9890241271)
(890,0.9890706212)
(900,0.9891051596)
(910,0.9891504323)
(920,0.9891861302)
(930,0.9892375991)
(940,0.9892665566)
(950,0.9892495561)
(960,0.9892098034)
(970,0.9891548716)
(980,0.9891232782)
(990,0.9891100809)
(1000,0.9891022922)
(1010,0.9891156711)
(1020,0.9891475824)
(1030,0.989182598)
(1040,0.9892077373)
(1050,0.9892306803)
(1060,0.9892303402)
(1070,0.9892120644)
(1080,0.9892520515)
(1090,0.9893770589)
(1100,0.9895450176)
(1110,0.9897216763)
(1120,0.989864802)
(1130,0.989862276)
(1140,0.9898732828)
(1150,0.9898897697)
(1160,0.9898958578)
(1170,0.9898994226)
(1180,0.9899111765)
(1190,0.9899258671)
(1200,0.9899381013)
(1210,0.9899638894)
(1220,0.9900086834)
(1230,0.9900510679)
(1240,0.9900909769)
(1250,0.9901284787)
(1260,0.9901581637)
(1270,0.9901907801)
(1280,0.9902182337)
(1290,0.9902513677)
(1300,0.9902765697)
(1310,0.9902938864)
(1320,0.9903250499)
(1330,0.9903455298)
(1340,0.9903552576)
(1350,0.9903705513)
(1360,0.9903833473)
(1370,0.9904017562)
(1380,0.9904203426)
(1390,0.9904335908)
(1400,0.9904387464)
(1410,0.9904440992)
(1420,0.9904440619)
(1430,0.9904468481)
(1440,0.9904442786)
(1450,0.990461195)
(1460,0.9904754226)
(1470,0.9904898678)
(1480,0.9905016383)
(1490,0.9905107249)
(1500,0.9905226769)
(1510,0.9905264276)
(1520,0.9905386346)
(1530,0.9905481459)
(1540,0.9905661965)
(1550,0.9905648195)
(1560,0.9905831373)
(1570,0.9905931862)
(1580,0.9905949404)
(1590,0.9906023886)
(1600,0.9906043677)
(1610,0.9906176745)
(1620,0.9906339406)
(1630,0.9906361954)
(1640,0.9906385871)
(1650,0.9906326106)
(1660,0.9906266495)
(1670,0.9906376669)
(1680,0.9906601577)
(1690,0.9906770786)
(1700,0.9907054514)
(1710,0.9907340619)
(1720,0.9907513626)
(1730,0.9907772633)
(1740,0.9907976775)
(1750,0.9908210155)
(1760,0.9908302333)
(1770,0.9908566646)
(1780,0.9908804039)
(1790,0.9909213586)
(1800,0.9909253134)
(1810,0.9909379808)
(1820,0.9909563996)
(1830,0.9909663369)
(1840,0.9909877963)
(1850,0.9909979572)
(1860,0.9910053246)
(1870,0.9910243666)
(1880,0.9910261638)
(1890,0.9910366724)
(1900,0.991044534)
(1910,0.9910524333)
(1920,0.9910545689)
(1930,0.9910597141)
(1940,0.9910447154)
(1950,0.9910297999)
(1960,0.9910033857)
(1970,0.9909856154)
(1980,0.9909621535)
(1990,0.9909300224)
(2000,0.990892176)
(2010,0.9908602245)
(2020,0.9908225002)
(2030,0.9908051015)
(2040,0.9907645891)
(2050,0.990735757)
(2060,0.9906691682)
(2070,0.9906346092)
(2080,0.9905594313)
(2090,0.9904959295)
(2100,0.9904295134)
(2110,0.9903455926)
(2120,0.9902587966)
(2130,0.9901224778)
(2140,0.9900153091)
(2150,0.9898877065)
(2160,0.9897455955)
(2170,0.9896152341)
(2180,0.9894527433)
(2190,0.9893252473)
(2200,0.9891540258)
(2210,0.9889915338)
(2220,0.9888349972)
(2230,0.9886667767)
(2240,0.9884984949)
(2250,0.9883243581)
(2260,0.9881532176)
(2270,0.9879792868)
(2280,0.987805166)
(2290,0.9876487814)
(2300,0.9875071972)
(2310,0.9873596418)
(2320,0.9872358401)
(2330,0.9871238422)
(2340,0.98700013)
(2350,0.9869233134)
(2360,0.9868380207)
(2370,0.9867646407)
(2380,0.9867088215)
(2390,0.9866768424)
(2400,0.9866243395)
(2410,0.9865896925)
(2420,0.9865638734)
(2430,0.9865499257)
(2440,0.9865684191)
(2450,0.9865636288)
(2460,0.9865793674)
(2470,0.986604234)
(2480,0.9866261848)
(2490,0.9866366478)
(2500,0.9866676937)};\label{plots:plot8}

==> charts/minimization_CIFAR.tex <==
\addplot[black] coordinates{(0,6.93893)
(10,6.93893)
(20,6.93893)
(30,6.93893)
(40,6.93893)
(50,6.93893)
(60,6.93893)
(70,6.93893)
(80,6.93893)
(90,6.93893)
(100,6.93893)
(110,6.93893)
(120,6.93893)
(130,6.93893)
(140,6.93893)
(150,6.93893)
(160,6.93893)
(170,6.93893)
(180,6.93893)
(190,6.93888)
(200,6.93857)
(210,6.93619)
(220,6.9201)
(230,6.85805)
(240,6.78079)
(250,6.72545)
(260,6.34152)
(270,6.06467)
(280,5.88498)
(290,5.72978)
(300,5.59859)
(310,5.49091)
(320,5.40295)
(330,5.32928)
(340,5.26534)
(350,5.20879)
(360,5.1581)
(370,5.11217)
(380,5.07027)
(390,5.03194)
(400,4.99658)
(410,4.96378)
(420,4.93333)
(430,4.90503)
(440,4.87867)
(450,4.85408)
(460,4.83095)
(470,4.8091)
(480,4.78836)
(490,4.76863)
(500,4.74968)
(510,4.73153)
(520,4.71433)
(530,4.69809)
(540,4.68274)
(550,4.66812)
(560,4.65414)
(570,4.64068)
(580,4.6278)
(590,4.61541)
(600,4.60352)
(610,4.59189)
(620,4.58077)
(630,4.57002)
(640,4.55968)
(650,4.54966)
(660,4.53996)
(670,4.53057)
(680,4.52148)
(690,4.51273)
(700,4.50428)
(710,4.49608)
(720,4.48805)
(730,4.48026)
(740,4.47268)
(750,4.46533)
(760,4.4582)
(770,4.45128)
(780,4.44453)
(790,4.43794)
(800,4.4315)
(810,4.42522)
(820,4.41911)
(830,4.41317)
(840,4.40732)
(850,4.40162)
(860,4.39608)
(870,4.39057)
(880,4.38518)
(890,4.37986)
(900,4.37467)
(910,4.36958)
(920,4.36456)
(930,4.35966)
(940,4.3548)
(950,4.35005)
(960,4.34539)
(970,4.34083)
(980,4.33633)
(990,4.33194)
(1000,4.32761)
(1010,4.32335)
(1020,4.31916)
(1030,4.31504)
(1040,4.31104)
(1050,4.30708)
(1060,4.30317)
(1070,4.29935)
(1080,4.29557)
(1090,4.29185)
(1100,4.28824)
(1110,4.28464)
(1120,4.28112)
(1130,4.27767)
(1140,4.27427)
(1150,4.27091)
(1160,4.26762)
(1170,4.26431)
(1180,4.26108)
(1190,4.25791)
(1200,4.25479)
(1210,4.25171)
(1220,4.24871)
(1230,4.24573)
(1240,4.24281)
(1250,4.23991)
(1260,4.23705)
(1270,4.23421)
(1280,4.23141)
(1290,4.22866)
(1300,4.22596)
(1310,4.22326)
(1320,4.22062)
(1330,4.21799)
(1340,4.21541)
(1350,4.21286)
(1360,4.21034)
(1370,4.20785)
(1380,4.2054)
(1390,4.20294)
(1400,4.20053)
(1410,4.19816)
(1420,4.19579)
(1430,4.19345)
(1440,4.19115)
(1450,4.1889)
(1460,4.18668)
(1470,4.18446)
(1480,4.18227)
(1490,4.18014)
(1500,4.17799)
(1510,4.17588)
(1520,4.17381)
(1530,4.17173)
(1540,4.16969)
(1550,4.16773)
(1560,4.16574)
(1570,4.1638)
(1580,4.16189)
(1590,4.15999)
(1600,4.15813)
(1610,4.15626)
(1620,4.15441)
(1630,4.1526)
(1640,4.15077)
(1650,4.149)
(1660,4.14727)
(1670,4.14552)
(1680,4.14381)
(1690,4.14215)
(1700,4.14048)
(1710,4.13884)
(1720,4.13722)
(1730,4.13561)
(1740,4.13404)
(1750,4.13247)
(1760,4.13087)
(1770,4.12928)
(1780,4.12775)
(1790,4.12622)
(1800,4.12474)
(1810,4.12324)
(1820,4.12181)
(1830,4.12038)
(1840,4.11897)
(1850,4.11756)
(1860,4.11619)
(1870,4.11483)
(1880,4.11352)
(1890,4.11222)
(1900,4.11091)
(1910,4.10962)
(1920,4.10831)
(1930,4.10704)
(1940,4.1058)
(1950,4.10457)
(1960,4.10338)
(1970,4.10218)
(1980,4.10099)
(1990,4.09982)
(2000,4.09869)
(2010,4.09755)
(2020,4.09642)
(2030,4.09533)
(2040,4.09423)
(2050,4.09316)
(2060,4.09212)
(2070,4.09108)
(2080,4.09008)
(2090,4.08907)
(2100,4.08813)
(2110,4.08718)
(2120,4.08627)
(2130,4.08533)
(2140,4.08444)
(2150,4.08358)
(2160,4.08273)
(2170,4.08193)
(2180,4.08112)
(2190,4.08036)
(2200,4.07959)
(2210,4.07887)
(2220,4.07815)
(2230,4.07742)
(2240,4.07674)
(2250,4.07605)
(2260,4.07533)
(2270,4.07465)
(2280,4.074)
(2290,4.07336)
(2300,4.07274)
(2310,4.07223)
(2320,4.07171)
(2330,4.07118)
(2340,4.07072)
(2350,4.07028)
(2360,4.06984)
(2370,4.06941)
(2380,4.069)
(2390,4.0686)
(2400,4.0682)
(2410,4.06785)
(2420,4.06747)
(2430,4.06711)
(2440,4.06675)
(2450,4.06641)
(2460,4.06612)
(2470,4.06584)
(2480,4.06552)
(2490,4.06526)
(2500,4.06504)};\label{plots:plot4}
\addplot[red] coordinates{(0,6.93893)
(10,6.93893)
(20,6.93893)
(30,6.93893)
(40,6.93893)
(50,6.93893)
(60,6.93893)
(70,6.93893)
(80,6.93893)
(90,6.93893)
(100,6.93893)
(110,6.93893)
(120,6.93893)
(130,6.93893)
(140,6.93893)
(150,6.93893)
(160,6.93893)
(170,6.93893)
(180,6.93893)
(190,6.93892)
(200,6.93884)
(210,6.93825)
(220,6.93399)
(230,6.90898)
(240,6.84093)
(250,6.76355)
(260,6.35418)
(270,6.0767)
(280,5.90358)
(290,5.74575)
(300,5.60521)
(310,5.49066)
(320,5.3997)
(330,5.32506)
(340,5.26173)
(350,5.20686)
(360,5.15824)
(370,5.11466)
(380,5.07548)
(390,5.04003)
(400,5.00753)
(410,4.9775)
(420,4.94957)
(430,4.92366)
(440,4.89942)
(450,4.87679)
(460,4.85564)
(470,4.83575)
(480,4.81702)
(490,4.79931)
(500,4.78256)
(510,4.76668)
(520,4.75131)
(530,4.73631)
(540,4.72212)
(550,4.70893)
(560,4.69652)
(570,4.68473)
(580,4.67336)
(590,4.66241)
(600,4.65195)
(610,4.64194)
(620,4.6323)
(630,4.623)
(640,4.61396)
(650,4.60515)
(660,4.59674)
(670,4.58849)
(680,4.58059)
(690,4.5729)
(700,4.56544)
(710,4.55826)
(720,4.55128)
(730,4.54447)
(740,4.53782)
(750,4.5314)
(760,4.52513)
(770,4.519)
(780,4.51306)
(790,4.50729)
(800,4.50166)
(810,4.49618)
(820,4.4908)
(830,4.48555)
(840,4.48038)
(850,4.47538)
(860,4.47045)
(870,4.46563)
(880,4.46087)
(890,4.45625)
(900,4.45174)
(910,4.44729)
(920,4.44293)
(930,4.43869)
(940,4.43452)
(950,4.43043)
(960,4.42643)
(970,4.42247)
(980,4.41861)
(990,4.41479)
(1000,4.41105)
(1010,4.4074)
(1020,4.40381)
(1030,4.4003)
(1040,4.39687)
(1050,4.39346)
(1060,4.39018)
(1070,4.3869)
(1080,4.3837)
(1090,4.38055)
(1100,4.37749)
(1110,4.37445)
(1120,4.37148)
(1130,4.36855)
(1140,4.36567)
(1150,4.36283)
(1160,4.36008)
(1170,4.35735)
(1180,4.35468)
(1190,4.35202)
(1200,4.3494)
(1210,4.34686)
(1220,4.34435)
(1230,4.34182)
(1240,4.33932)
(1250,4.33689)
(1260,4.33448)
(1270,4.33209)
(1280,4.32972)
(1290,4.32741)
(1300,4.32509)
(1310,4.32287)
(1320,4.32063)
(1330,4.31843)
(1340,4.31627)
(1350,4.31413)
(1360,4.31203)
(1370,4.30996)
(1380,4.30793)
(1390,4.30589)
(1400,4.30389)
(1410,4.30187)
(1420,4.29994)
(1430,4.29802)
(1440,4.29608)
(1450,4.2942)
(1460,4.29235)
(1470,4.29049)
(1480,4.28868)
(1490,4.2869)
(1500,4.28513)
(1510,4.28338)
(1520,4.28167)
(1530,4.27998)
(1540,4.2783)
(1550,4.27665)
(1560,4.27501)
(1570,4.27342)
(1580,4.27187)
(1590,4.27034)
(1600,4.2688)
(1610,4.26727)
(1620,4.26577)
(1630,4.26429)
(1640,4.26283)
(1650,4.26137)
(1660,4.25996)
(1670,4.25857)
(1680,4.2572)
(1690,4.25585)
(1700,4.25448)
(1710,4.25314)
(1720,4.2518)
(1730,4.25051)
(1740,4.24923)
(1750,4.24796)
(1760,4.24669)
(1770,4.24544)
(1780,4.24423)
(1790,4.24301)
(1800,4.2418)
(1810,4.24063)
(1820,4.23948)
(1830,4.23833)
(1840,4.23722)
(1850,4.23609)
(1860,4.23499)
(1870,4.2339)
(1880,4.23285)
(1890,4.23183)
(1900,4.23079)
(1910,4.2298)
(1920,4.22879)
(1930,4.2278)
(1940,4.22682)
(1950,4.22588)
(1960,4.22494)
(1970,4.224)
(1980,4.2231)
(1990,4.22223)
(2000,4.22133)
(2010,4.22045)
(2020,4.21963)
(2030,4.21883)
(2040,4.21801)
(2050,4.21721)
(2060,4.21643)
(2070,4.21562)
(2080,4.21487)
(2090,4.21413)
(2100,4.21338)
(2110,4.21263)
(2120,4.21194)
(2130,4.21125)
(2140,4.21055)
(2150,4.20987)
(2160,4.20919)
(2170,4.20851)
(2180,4.20784)
(2190,4.20719)
(2200,4.20655)
(2210,4.2059)
(2220,4.20525)
(2230,4.20461)
(2240,4.204)
(2250,4.20337)
(2260,4.20276)
(2270,4.20217)
(2280,4.20157)
(2290,4.201)
(2300,4.20044)
(2310,4.19987)
(2320,4.19929)
(2330,4.19867)
(2340,4.19812)
(2350,4.19756)
(2360,4.197)
(2370,4.19649)
(2380,4.19595)
(2390,4.19546)
(2400,4.19496)
(2410,4.19446)
(2420,4.19396)
(2430,4.19344)
(2440,4.19296)
(2450,4.19247)
(2460,4.19197)
(2470,4.19149)
(2480,4.19102)
(2490,4.19054)
(2500,4.19008)};\label{plots:plot1}
\addplot[green] coordinates{(0,6.93893)
(10,6.93893)
(20,6.93893)
(30,6.93893)
(40,6.93893)
(50,6.93893)
(60,6.93893)
(70,6.93893)
(80,6.93893)
(90,6.93893)
(100,6.93893)
(110,6.93893)
(120,6.93893)
(130,6.93893)
(140,6.93893)
(150,6.93893)
(160,6.93893)
(170,6.93893)
(180,6.93893)
(190,6.93893)
(200,6.93891)
(210,6.9388)
(220,6.93807)
(230,6.93356)
(240,6.91094)
(250,6.8433)
(260,6.40348)
(270,6.09985)
(280,5.91493)
(290,5.76161)
(300,5.63598)
(310,5.53583)
(320,5.45614)
(330,5.39053)
(340,5.33491)
(350,5.28661)
(360,5.24363)
(370,5.2047)
(380,5.16922)
(390,5.13644)
(400,5.10576)
(410,5.07732)
(420,5.05095)
(430,5.02623)
(440,5.00284)
(450,4.98155)
(460,4.96197)
(470,4.94336)
(480,4.92579)
(490,4.90905)
(500,4.89316)
(510,4.87812)
(520,4.86373)
(530,4.85009)
(540,4.83725)
(550,4.82524)
(560,4.81393)
(570,4.80297)
(580,4.79237)
(590,4.78223)
(600,4.77253)
(610,4.76324)
(620,4.75436)
(630,4.74584)
(640,4.73762)
(650,4.72971)
(660,4.72207)
(670,4.71474)
(680,4.70762)
(690,4.70075)
(700,4.69406)
(710,4.68755)
(720,4.68129)
(730,4.6752)
(740,4.66934)
(750,4.66363)
(760,4.65815)
(770,4.65279)
(780,4.64756)
(790,4.64249)
(800,4.63757)
(810,4.63277)
(820,4.62811)
(830,4.62359)
(840,4.61922)
(850,4.61501)
(860,4.6109)
(870,4.60698)
(880,4.60259)
(890,4.59836)
(900,4.59421)
(910,4.59016)
(920,4.58624)
(930,4.58242)
(940,4.57864)
(950,4.57496)
(960,4.57133)
(970,4.5678)
(980,4.56434)
(990,4.56097)
(1000,4.55768)
(1010,4.5545)
(1020,4.55139)
(1030,4.54824)
(1040,4.54516)
(1050,4.54216)
(1060,4.5392)
(1070,4.53633)
(1080,4.53353)
(1090,4.53079)
(1100,4.52808)
(1110,4.52544)
(1120,4.52285)
(1130,4.52032)
(1140,4.51784)
(1150,4.51541)
(1160,4.51301)
(1170,4.51066)
(1180,4.50835)
(1190,4.50602)
(1200,4.50375)
(1210,4.50153)
(1220,4.49932)
(1230,4.49717)
(1240,4.49505)
(1250,4.49301)
(1260,4.49097)
(1270,4.48892)
(1280,4.48686)
(1290,4.48487)
(1300,4.48291)
(1310,4.48096)
(1320,4.47904)
(1330,4.47714)
(1340,4.47529)
(1350,4.47347)
(1360,4.47173)
(1370,4.46996)
(1380,4.46816)
(1390,4.46639)
(1400,4.46464)
(1410,4.46287)
(1420,4.46118)
(1430,4.45949)
(1440,4.4578)
(1450,4.45615)
(1460,4.45456)
(1470,4.45298)
(1480,4.45144)
(1490,4.44996)
(1500,4.44845)
(1510,4.44698)
(1520,4.44558)
(1530,4.44414)
(1540,4.4427)
(1550,4.4413)
(1560,4.43992)
(1570,4.43855)
(1580,4.43721)
(1590,4.4359)
(1600,4.43461)
(1610,4.43329)
(1620,4.432)
(1630,4.43072)
(1640,4.42945)
(1650,4.42819)
(1660,4.42696)
(1670,4.42575)
(1680,4.42453)
(1690,4.42333)
(1700,4.42216)
(1710,4.42099)
(1720,4.41983)
(1730,4.41867)
(1740,4.41755)
(1750,4.41642)
(1760,4.41529)
(1770,4.4142)
(1780,4.41313)
(1790,4.41204)
(1800,4.411)
(1810,4.40997)
(1820,4.40893)
(1830,4.40794)
(1840,4.40696)
(1850,4.40598)
(1860,4.40499)
(1870,4.40399)
(1880,4.40303)
(1890,4.40209)
(1900,4.40117)
(1910,4.40024)
(1920,4.39934)
(1930,4.39844)
(1940,4.39755)
(1950,4.39671)
(1960,4.39583)
(1970,4.39499)
(1980,4.39413)
(1990,4.39333)
(2000,4.39249)
(2010,4.39168)
(2020,4.39086)
(2030,4.39004)
(2040,4.38927)
(2050,4.38848)
(2060,4.38775)
(2070,4.38702)
(2080,4.38633)
(2090,4.38565)
(2100,4.38495)
(2110,4.38429)
(2120,4.3836)
(2130,4.38295)
(2140,4.38228)
(2150,4.3816)
(2160,4.38096)
(2170,4.38032)
(2180,4.37969)
(2190,4.37906)
(2200,4.37846)
(2210,4.37785)
(2220,4.37726)
(2230,4.37668)
(2240,4.37611)
(2250,4.37555)
(2260,4.37501)
(2270,4.37448)
(2280,4.37396)
(2290,4.37345)
(2300,4.37296)
(2310,4.37248)
(2320,4.37199)
(2330,4.37156)
(2340,4.37112)
(2350,4.37055)
(2360,4.37)
(2370,4.36948)
(2380,4.36895)
(2390,4.36846)
(2400,4.36798)
(2410,4.3675)
(2420,4.36703)
(2430,4.36654)
(2440,4.36612)
(2450,4.36572)
(2460,4.3653)
(2470,4.36492)
(2480,4.36457)
(2490,4.3642)
(2500,4.36385)};\label{plots:plot2}
\addplot[blue] coordinates{(0,6.93893)
(10,6.93893)
(20,6.93893)
(30,6.93893)
(40,6.93893)
(50,6.93893)
(60,6.93893)
(70,6.93893)
(80,6.93893)
(90,6.93893)
(100,6.93893)
(110,6.93893)
(120,6.93893)
(130,6.93893)
(140,6.93893)
(150,6.93893)
(160,6.93893)
(170,6.93893)
(180,6.93893)
(190,6.93893)
(200,6.93893)
(210,6.93893)
(220,6.93893)
(230,6.93893)
(240,6.93893)
(250,6.93893)
(260,6.93871)
(270,6.87595)
(280,6.39941)
(290,6.07891)
(300,5.8783)
(310,5.73433)
(320,5.63656)
(330,5.56743)
(340,5.51337)
(350,5.46906)
(360,5.43142)
(370,5.39842)
(380,5.36933)
(390,5.34319)
(400,5.3194)
(410,5.29749)
(420,5.27725)
(430,5.25837)
(440,5.24064)
(450,5.22421)
(460,5.20889)
(470,5.19452)
(480,5.18094)
(490,5.16817)
(500,5.15616)
(510,5.14498)
(520,5.13445)
(530,5.12457)
(540,5.11527)
(550,5.10651)
(560,5.0982)
(570,5.09037)
(580,5.0829)
(590,5.07581)
(600,5.06893)
(610,5.06237)
(620,5.05601)
(630,5.04999)
(640,5.04424)
(650,5.0388)
(660,5.03364)
(670,5.02872)
(680,5.02404)
(690,5.01949)
(700,5.01509)
(710,5.01087)
(720,5.00683)
(730,5.00297)
(740,4.99927)
(750,4.99574)
(760,4.99231)
(770,4.98897)
(780,4.98573)
(790,4.98258)
(800,4.97948)
(810,4.97649)
(820,4.97357)
(830,4.97076)
(840,4.96806)
(850,4.9654)
(860,4.96273)
(870,4.96013)
(880,4.9576)
(890,4.95511)
(900,4.95274)
(910,4.95045)
(920,4.94822)
(930,4.94605)
(940,4.94395)
(950,4.9419)
(960,4.9399)
(970,4.93797)
(980,4.93616)
(990,4.93442)
(1000,4.93271)
(1010,4.9311)
(1020,4.92941)
(1030,4.92774)
(1040,4.92602)
(1050,4.92435)
(1060,4.92269)
(1070,4.9211)
(1080,4.91955)
(1090,4.91802)
(1100,4.91652)
(1110,4.91508)
(1120,4.91366)
(1130,4.91226)
(1140,4.91091)
(1150,4.9096)
(1160,4.90827)
(1170,4.90694)
(1180,4.90563)
(1190,4.90437)
(1200,4.90314)
(1210,4.90195)
(1220,4.90081)
(1230,4.8997)
(1240,4.89859)
(1250,4.89749)
(1260,4.8964)
(1270,4.89533)
(1280,4.89431)
(1290,4.89327)
(1300,4.89229)
(1310,4.89128)
(1320,4.89032)
(1330,4.88938)
(1340,4.88845)
(1350,4.88752)
(1360,4.88659)
(1370,4.88569)
(1380,4.8848)
(1390,4.88392)
(1400,4.88307)
(1410,4.88221)
(1420,4.88142)
(1430,4.88064)
(1440,4.87989)
(1450,4.87916)
(1460,4.8784)
(1470,4.87765)
(1480,4.87693)
(1490,4.87619)
(1500,4.87548)
(1510,4.87479)
(1520,4.87412)
(1530,4.87346)
(1540,4.87281)
(1550,4.87219)
(1560,4.87156)
(1570,4.87093)
(1580,4.87033)
(1590,4.86975)
(1600,4.86917)
(1610,4.86855)
(1620,4.86801)
(1630,4.86742)
(1640,4.86688)
(1650,4.8663)
(1660,4.86573)
(1670,4.86519)
(1680,4.86466)
(1690,4.86411)
(1700,4.86358)
(1710,4.86309)
(1720,4.86257)
(1730,4.86206)
(1740,4.86156)
(1750,4.86108)
(1760,4.86058)
(1770,4.86013)
(1780,4.85965)
(1790,4.85921)
(1800,4.85873)
(1810,4.85829)
(1820,4.85784)
(1830,4.85742)
(1840,4.85698)
(1850,4.85655)
(1860,4.85613)
(1870,4.8557)
(1880,4.85527)
(1890,4.85488)
(1900,4.8545)
(1910,4.85409)
(1920,4.8537)
(1930,4.85332)
(1940,4.85295)
(1950,4.85256)
(1960,4.8522)
(1970,4.85185)
(1980,4.85152)
(1990,4.85119)
(2000,4.85087)
(2010,4.85054)
(2020,4.85025)
(2030,4.84995)
(2040,4.84968)
(2050,4.84942)
(2060,4.84918)
(2070,4.84894)
(2080,4.8487)
(2090,4.84842)
(2100,4.84817)
(2110,4.84792)
(2120,4.84767)
(2130,4.84743)
(2140,4.8472)
(2150,4.84696)
(2160,4.84673)
(2170,4.84649)
(2180,4.84628)
(2190,4.84605)
(2200,4.84582)
(2210,4.8456)
(2220,4.84538)
(2230,4.84517)
(2240,4.84495)
(2250,4.84474)
(2260,4.84453)
(2270,4.84432)
(2280,4.84409)
(2290,4.84388)
(2300,4.84366)
(2310,4.84345)
(2320,4.84325)
(2330,4.84304)
(2340,4.84282)
(2350,4.84263)
(2360,4.84245)
(2370,4.84228)
(2380,4.84213)
(2390,4.84198)
(2400,4.84184)
(2410,4.84172)
(2420,4.84157)
(2430,4.84146)
(2440,4.84133)
(2450,4.84121)
(2460,4.84108)
(2470,4.84094)
(2480,4.84081)
(2490,4.84068)
(2500,4.84056)};\label{plots:plot3}

==> charts/minimization_MNIST.tex <==
\addplot[black] coordinates{
(0,6.29604)
(10,6.29604)
(20,6.29604)
(30,6.29604)
(40,6.29604)
(50,6.29604)
(60,6.29604)
(70,6.29604)
(80,6.29604)
(90,6.29596)
(100,6.29294)
(110,6.20346)
(120,5.86785)
(130,5.66296)
(140,5.55218)
(150,5.48307)
(160,5.43735)
(170,5.40787)
(180,5.38891)
(190,5.37667)
(200,5.36867)
(210,5.36332)
(220,5.35964)
(230,5.35702)
(240,5.35522)
(250,5.33396)
(260,4.81219)
(270,4.41029)
(280,4.15975)
(290,3.98436)
(300,3.85016)
(310,3.73806)
(320,3.64322)
(330,3.56164)
(340,3.49011)
(350,3.42617)
(360,3.36837)
(370,3.31612)
(380,3.26847)
(390,3.22481)
(400,3.18419)
(410,3.14635)
(420,3.11105)
(430,3.07794)
(440,3.04685)
(450,3.01755)
(460,2.99006)
(470,2.9641)
(480,2.93963)
(490,2.91642)
(500,2.89435)
(510,2.87333)
(520,2.85319)
(530,2.83407)
(540,2.81569)
(550,2.79812)
(560,2.78129)
(570,2.76504)
(580,2.74946)
(590,2.73443)
(600,2.71993)
(610,2.70588)
(620,2.69241)
(630,2.67935)
(640,2.66668)
(650,2.65444)
(660,2.64254)
(670,2.631)
(680,2.61984)
(690,2.60888)
(700,2.59836)
(710,2.58827)
(720,2.57837)
(730,2.5688)
(740,2.55941)
(750,2.55018)
(760,2.54125)
(770,2.53263)
(780,2.52425)
(790,2.51611)
(800,2.50813)
(810,2.50036)
(820,2.49281)
(830,2.48546)
(840,2.47832)
(850,2.47129)
(860,2.4645)
(870,2.45779)
(880,2.45127)
(890,2.44498)
(900,2.43888)
(910,2.4329)
(920,2.42709)
(930,2.42141)
(940,2.41593)
(950,2.41056)
(960,2.40539)
(970,2.40033)
(980,2.39541)
(990,2.39058)
(1000,2.38599)
(1010,2.38144)
(1020,2.37696)
(1030,2.37274)
(1040,2.36869)
(1050,2.36472)
(1060,2.36087)
(1070,2.35716)
(1080,2.35362)
(1090,2.35027)
(1100,2.34706)
(1110,2.34395)
(1120,2.34097)
(1130,2.33801)
(1140,2.33519)
(1150,2.33233)
(1160,2.32946)
(1170,2.3267)
(1180,2.32399)
(1190,2.32133)
(1200,2.31889)
(1210,2.31658)
(1220,2.31425)
(1230,2.31205)
(1240,2.3099)
(1250,2.3078)
(1260,2.30579)
(1270,2.30381)
(1280,2.30198)
(1290,2.30027)
(1300,2.29858)
(1310,2.29704)
(1320,2.29546)
(1330,2.29397)
(1340,2.29257)
(1350,2.29124)
(1360,2.28985)
(1370,2.28848)
(1380,2.28721)
(1390,2.28595)
(1400,2.28467)
(1410,2.28346)
(1420,2.28237)
(1430,2.2812)
(1440,2.28015)
(1450,2.2791)
(1460,2.27803)
(1470,2.27703)
(1480,2.27603)
(1490,2.27502)
(1500,2.27405)
(1510,2.27305)
(1520,2.27203)
(1530,2.27106)
(1540,2.27009)
(1550,2.26917)
(1560,2.26827)
(1570,2.26738)
(1580,2.2665)
(1590,2.26565)
(1600,2.26469)
(1610,2.26387)
(1620,2.26298)
(1630,2.26209)
(1640,2.26127)
(1650,2.26041)
(1660,2.25955)
(1670,2.2587)
(1680,2.25789)
(1690,2.25709)
(1700,2.2563)
(1710,2.25548)
(1720,2.25468)
(1730,2.2539)
(1740,2.25312)
(1750,2.25229)
(1760,2.2515)
(1770,2.25068)
(1780,2.24988)
(1790,2.2491)
(1800,2.24833)
(1810,2.2475)
(1820,2.24669)
(1830,2.24592)
(1840,2.24511)
(1850,2.24433)
(1860,2.24352)
(1870,2.24272)
(1880,2.24193)
(1890,2.24113)
(1900,2.24031)
(1910,2.2395)
(1920,2.23866)
(1930,2.23788)
(1940,2.23706)
(1950,2.23628)
(1960,2.23549)
(1970,2.23478)
(1980,2.23395)
(1990,2.23322)
(2000,2.23237)
(2010,2.23161)
(2020,2.23083)
(2030,2.23009)
(2040,2.22935)
(2050,2.22863)
(2060,2.22783)
(2070,2.2271)
(2080,2.22638)
(2090,2.22567)
(2100,2.22496)
(2110,2.2242)
(2120,2.22346)
(2130,2.22271)
(2140,2.222)
(2150,2.22134)
(2160,2.22056)
(2170,2.21987)
(2180,2.21916)
(2190,2.21849)
(2200,2.21786)
(2210,2.21722)
(2220,2.21656)
(2230,2.21593)
(2240,2.21526)
(2250,2.21468)
(2260,2.21405)
(2270,2.21342)
(2280,2.2128)
(2290,2.21219)
(2300,2.21154)
(2310,2.21092)
(2320,2.2103)
(2330,2.20971)
(2340,2.20915)
(2350,2.20861)
(2360,2.20811)
(2370,2.20768)
(2380,2.20714)
(2390,2.20663)
(2400,2.20608)
(2410,2.20554)
(2420,2.20499)
(2430,2.2045)
(2440,2.20397)
(2450,2.20343)
(2460,2.20291)
(2470,2.20239)
(2480,2.20186)
(2490,2.20133)
(2500,2.20086)};\label{plots:plot4}
\addplot[red] coordinates{
(0,6.29604)
(10,6.29604)
(20,6.29604)
(30,6.29604)
(40,6.29604)
(50,6.29604)
(60,6.29604)
(70,6.29604)
(80,6.29604)
(90,6.29598)
(100,6.29386)
(110,6.22794)
(120,5.91432)
(130,5.70155)
(140,5.59416)
(150,5.53072)
(160,5.48769)
(170,5.45887)
(180,5.44003)
(190,5.42805)
(200,5.4204)
(210,5.41547)
(220,5.41225)
(230,5.41018)
(240,5.4088)
(250,5.38658)
(260,4.83788)
(270,4.42213)
(280,4.16584)
(290,3.98777)
(300,3.85254)
(310,3.742)
(320,3.6472)
(330,3.56512)
(340,3.49321)
(350,3.4291)
(360,3.37146)
(370,3.31921)
(380,3.27139)
(390,3.22761)
(400,3.18709)
(410,3.14939)
(420,3.11431)
(430,3.08147)
(440,3.05068)
(450,3.0218)
(460,2.99452)
(470,2.96882)
(480,2.9444)
(490,2.92117)
(500,2.89913)
(510,2.8782)
(520,2.85826)
(530,2.8392)
(540,2.82097)
(550,2.80344)
(560,2.78668)
(570,2.77064)
(580,2.75521)
(590,2.74036)
(600,2.7261)
(610,2.71217)
(620,2.69875)
(630,2.68582)
(640,2.67341)
(650,2.66135)
(660,2.64958)
(670,2.6382)
(680,2.62708)
(690,2.61627)
(700,2.60592)
(710,2.59577)
(720,2.58591)
(730,2.57634)
(740,2.56707)
(750,2.55805)
(760,2.5493)
(770,2.54073)
(780,2.53246)
(790,2.52435)
(800,2.51655)
(810,2.5089)
(820,2.50145)
(830,2.49425)
(840,2.48722)
(850,2.48039)
(860,2.47377)
(870,2.46728)
(880,2.46087)
(890,2.45478)
(900,2.44877)
(910,2.44291)
(920,2.43706)
(930,2.43148)
(940,2.42609)
(950,2.42077)
(960,2.41563)
(970,2.41063)
(980,2.4058)
(990,2.40099)
(1000,2.39627)
(1010,2.39178)
(1020,2.38743)
(1030,2.38315)
(1040,2.37906)
(1050,2.37504)
(1060,2.3712)
(1070,2.36746)
(1080,2.36376)
(1090,2.36021)
(1100,2.35685)
(1110,2.35352)
(1120,2.35035)
(1130,2.34723)
(1140,2.34413)
(1150,2.34125)
(1160,2.33845)
(1170,2.33585)
(1180,2.33325)
(1190,2.33078)
(1200,2.32842)
(1210,2.3262)
(1220,2.32402)
(1230,2.32193)
(1240,2.31983)
(1250,2.31793)
(1260,2.31605)
(1270,2.31423)
(1280,2.31243)
(1290,2.31078)
(1300,2.30914)
(1310,2.30757)
(1320,2.30604)
(1330,2.30463)
(1340,2.30324)
(1350,2.30185)
(1360,2.30068)
(1370,2.29955)
(1380,2.29833)
(1390,2.29722)
(1400,2.2961)
(1410,2.29496)
(1420,2.29401)
(1430,2.29295)
(1440,2.29196)
(1450,2.29094)
(1460,2.28998)
(1470,2.28902)
(1480,2.288)
(1490,2.28711)
(1500,2.28611)
(1510,2.28507)
(1520,2.28409)
(1530,2.28309)
(1540,2.28209)
(1550,2.28112)
(1560,2.28015)
(1570,2.27925)
(1580,2.27828)
(1590,2.27739)
(1600,2.27652)
(1610,2.27561)
(1620,2.27467)
(1630,2.27378)
(1640,2.27289)
(1650,2.27201)
(1660,2.27117)
(1670,2.27027)
(1680,2.26932)
(1690,2.26844)
(1700,2.26766)
(1710,2.26682)
(1720,2.26595)
(1730,2.26519)
(1740,2.26428)
(1750,2.26342)
(1760,2.26254)
(1770,2.26171)
(1780,2.26084)
(1790,2.26007)
(1800,2.25929)
(1810,2.25848)
(1820,2.25772)
(1830,2.257)
(1840,2.25621)
(1850,2.2553)
(1860,2.25452)
(1870,2.25374)
(1880,2.25299)
(1890,2.25217)
(1900,2.2515)
(1910,2.25079)
(1920,2.25006)
(1930,2.24935)
(1940,2.24862)
(1950,2.24789)
(1960,2.24717)
(1970,2.24646)
(1980,2.24574)
(1990,2.24502)
(2000,2.24428)
(2010,2.24366)
(2020,2.24302)
(2030,2.24232)
(2040,2.24165)
(2050,2.24105)
(2060,2.24042)
(2070,2.23981)
(2080,2.2392)
(2090,2.23853)
(2100,2.23795)
(2110,2.23735)
(2120,2.2368)
(2130,2.23625)
(2140,2.23571)
(2150,2.23515)
(2160,2.23466)
(2170,2.23402)
(2180,2.23347)
(2190,2.23299)
(2200,2.23244)
(2210,2.23187)
(2220,2.23133)
(2230,2.23078)
(2240,2.23021)
(2250,2.22973)
(2260,2.22918)
(2270,2.22859)
(2280,2.22805)
(2290,2.22757)
(2300,2.22706)
(2310,2.22655)
(2320,2.22599)
(2330,2.22545)
(2340,2.22492)
(2350,2.22445)
(2360,2.22396)
(2370,2.22347)
(2380,2.22297)
(2390,2.22252)
(2400,2.22213)
(2410,2.22166)
(2420,2.22125)
(2430,2.22084)
(2440,2.22039)
(2450,2.21994)
(2460,2.21951)
(2470,2.21909)
(2480,2.21863)
(2490,2.21821)
(2500,2.21777)};\label{plots:plot1}
\addplot[green] coordinates{
(0,6.29604)
(10,6.29604)
(20,6.29604)
(30,6.29604)
(40,6.29604)
(50,6.29604)
(60,6.29604)
(70,6.29604)
(80,6.29604)
(90,6.29602)
(100,6.29528)
(110,6.27103)
(120,6.05597)
(130,5.81227)
(140,5.70023)
(150,5.64307)
(160,5.60938)
(170,5.58645)
(180,5.57185)
(190,5.56281)
(200,5.55724)
(210,5.55386)
(220,5.55181)
(230,5.55058)
(240,5.54988)
(250,5.52515)
(260,4.90934)
(270,4.47425)
(280,4.21201)
(290,4.03126)
(300,3.89178)
(310,3.77929)
(320,3.68551)
(330,3.6035)
(340,3.53156)
(350,3.46732)
(360,3.40942)
(370,3.35715)
(380,3.30938)
(390,3.26538)
(400,3.22453)
(410,3.1866)
(420,3.15115)
(430,3.11811)
(440,3.08697)
(450,3.05771)
(460,3.0302)
(470,3.00426)
(480,2.97974)
(490,2.95642)
(500,2.93433)
(510,2.91316)
(520,2.89305)
(530,2.874)
(540,2.85586)
(550,2.83847)
(560,2.8218)
(570,2.80569)
(580,2.7903)
(590,2.77541)
(600,2.76114)
(610,2.74737)
(620,2.73416)
(630,2.72153)
(640,2.70923)
(650,2.69733)
(660,2.68579)
(670,2.67459)
(680,2.66386)
(690,2.65339)
(700,2.64331)
(710,2.63351)
(720,2.62396)
(730,2.61464)
(740,2.60558)
(750,2.59678)
(760,2.58817)
(770,2.57977)
(780,2.57171)
(790,2.56375)
(800,2.55604)
(810,2.54856)
(820,2.54131)
(830,2.53425)
(840,2.52732)
(850,2.52061)
(860,2.51405)
(870,2.50762)
(880,2.50136)
(890,2.49527)
(900,2.48928)
(910,2.48337)
(920,2.47759)
(930,2.47193)
(940,2.46646)
(950,2.46107)
(960,2.45576)
(970,2.4506)
(980,2.44552)
(990,2.44063)
(1000,2.43578)
(1010,2.43106)
(1020,2.42638)
(1030,2.42181)
(1040,2.41743)
(1050,2.41309)
(1060,2.40887)
(1070,2.40482)
(1080,2.4009)
(1090,2.39705)
(1100,2.39327)
(1110,2.38966)
(1120,2.38612)
(1130,2.38267)
(1140,2.37935)
(1150,2.37611)
(1160,2.37296)
(1170,2.36993)
(1180,2.36697)
(1190,2.36416)
(1200,2.36151)
(1210,2.35886)
(1220,2.35637)
(1230,2.354)
(1240,2.35165)
(1250,2.3495)
(1260,2.34742)
(1270,2.34532)
(1280,2.34344)
(1290,2.34165)
(1300,2.33987)
(1310,2.33817)
(1320,2.33652)
(1330,2.33496)
(1340,2.33344)
(1350,2.33197)
(1360,2.33053)
(1370,2.32912)
(1380,2.32782)
(1390,2.32655)
(1400,2.32538)
(1410,2.32422)
(1420,2.32309)
(1430,2.32207)
(1440,2.32099)
(1450,2.31995)
(1460,2.31888)
(1470,2.31782)
(1480,2.31674)
(1490,2.31577)
(1500,2.31477)
(1510,2.31383)
(1520,2.31288)
(1530,2.31196)
(1540,2.31098)
(1550,2.31003)
(1560,2.30914)
(1570,2.30821)
(1580,2.30733)
(1590,2.30647)
(1600,2.30562)
(1610,2.30478)
(1620,2.30398)
(1630,2.30317)
(1640,2.30236)
(1650,2.30156)
(1660,2.30081)
(1670,2.30007)
(1680,2.29935)
(1690,2.29858)
(1700,2.29785)
(1710,2.297)
(1720,2.2962)
(1730,2.29536)
(1740,2.29454)
(1750,2.29366)
(1760,2.29282)
(1770,2.29204)
(1780,2.29122)
(1790,2.29046)
(1800,2.28972)
(1810,2.28896)
(1820,2.28818)
(1830,2.28743)
(1840,2.28669)
(1850,2.28595)
(1860,2.2852)
(1870,2.28444)
(1880,2.28367)
(1890,2.28296)
(1900,2.2823)
(1910,2.28158)
(1920,2.28087)
(1930,2.28014)
(1940,2.27948)
(1950,2.27878)
(1960,2.27815)
(1970,2.27743)
(1980,2.27674)
(1990,2.2761)
(2000,2.27538)
(2010,2.2747)
(2020,2.27405)
(2030,2.27335)
(2040,2.27271)
(2050,2.27204)
(2060,2.27146)
(2070,2.27083)
(2080,2.27014)
(2090,2.26949)
(2100,2.2689)
(2110,2.26827)
(2120,2.26765)
(2130,2.26702)
(2140,2.26639)
(2150,2.26584)
(2160,2.26527)
(2170,2.26472)
(2180,2.26421)
(2190,2.26368)
(2200,2.2631)
(2210,2.26257)
(2220,2.26203)
(2230,2.26152)
(2240,2.26098)
(2250,2.26044)
(2260,2.25991)
(2270,2.25938)
(2280,2.25883)
(2290,2.25829)
(2300,2.25777)
(2310,2.25722)
(2320,2.25674)
(2330,2.25622)
(2340,2.2557)
(2350,2.25515)
(2360,2.25466)
(2370,2.25414)
(2380,2.25367)
(2390,2.25316)
(2400,2.25273)
(2410,2.25228)
(2420,2.25182)
(2430,2.25136)
(2440,2.2509)
(2450,2.25039)
(2460,2.24993)
(2470,2.24947)
(2480,2.24903)
(2490,2.24859)
(2500,2.24816)};\label{plots:plot2}
\addplot[blue] coordinates{
(0,6.29604)
(10,6.29604)
(20,6.29604)
(30,6.29604)
(40,6.29604)
(50,6.29604)
(60,6.29604)
(70,6.29604)
(80,6.29604)
(90,6.29604)
(100,6.29604)
(110,6.29604)
(120,6.29603)
(130,6.29592)
(140,6.29463)
(150,6.28194)
(160,6.23435)
(170,6.18243)
(180,6.14832)
(190,6.12708)
(200,6.11423)
(210,6.10745)
(220,6.10445)
(230,6.10331)
(240,6.10288)
(250,6.07698)
(260,5.29201)
(270,4.75493)
(280,4.46321)
(290,4.2711)
(300,4.12861)
(310,4.01323)
(320,3.91679)
(330,3.83421)
(340,3.76217)
(350,3.69835)
(360,3.64132)
(370,3.59001)
(380,3.54375)
(390,3.50181)
(400,3.46308)
(410,3.42749)
(420,3.39451)
(430,3.3638)
(440,3.33499)
(450,3.30798)
(460,3.2824)
(470,3.25837)
(480,3.23568)
(490,3.21432)
(500,3.19409)
(510,3.17471)
(520,3.15619)
(530,3.13841)
(540,3.12153)
(550,3.1054)
(560,3.08996)
(570,3.07519)
(580,3.06094)
(590,3.04719)
(600,3.03402)
(610,3.02149)
(620,3.00948)
(630,2.99793)
(640,2.98682)
(650,2.97614)
(660,2.96573)
(670,2.95571)
(680,2.94601)
(690,2.93664)
(700,2.92752)
(710,2.91875)
(720,2.91017)
(730,2.90184)
(740,2.89378)
(750,2.88593)
(760,2.8783)
(770,2.87088)
(780,2.86387)
(790,2.85704)
(800,2.85038)
(810,2.84393)
(820,2.83758)
(830,2.83146)
(840,2.82551)
(850,2.81973)
(860,2.81409)
(870,2.80859)
(880,2.80326)
(890,2.79799)
(900,2.79295)
(910,2.78801)
(920,2.7831)
(930,2.77837)
(940,2.77378)
(950,2.76929)
(960,2.76487)
(970,2.76063)
(980,2.75638)
(990,2.75226)
(1000,2.74823)
(1010,2.74436)
(1020,2.74072)
(1030,2.73729)
(1040,2.73393)
(1050,2.7308)
(1060,2.72766)
(1070,2.72458)
(1080,2.72172)
(1090,2.71893)
(1100,2.7162)
(1110,2.71355)
(1120,2.71102)
(1130,2.70854)
(1140,2.70602)
(1150,2.70371)
(1160,2.70135)
(1170,2.69905)
(1180,2.69682)
(1190,2.69461)
(1200,2.6924)
(1210,2.69029)
(1220,2.6883)
(1230,2.68633)
(1240,2.68451)
(1250,2.68267)
(1260,2.68103)
(1270,2.67934)
(1280,2.67776)
(1290,2.67617)
(1300,2.67461)
(1310,2.67308)
(1320,2.67171)
(1330,2.67028)
(1340,2.6689)
(1350,2.6676)
(1360,2.6662)
(1370,2.66499)
(1380,2.66376)
(1390,2.66254)
(1400,2.66143)
(1410,2.66036)
(1420,2.65924)
(1430,2.65819)
(1440,2.65718)
(1450,2.65621)
(1460,2.65516)
(1470,2.65421)
(1480,2.65338)
(1490,2.65251)
(1500,2.65167)
(1510,2.65093)
(1520,2.65014)
(1530,2.64941)
(1540,2.64867)
(1550,2.64793)
(1560,2.64718)
(1570,2.64641)
(1580,2.64569)
(1590,2.64496)
(1600,2.64429)
(1610,2.64356)
(1620,2.64291)
(1630,2.64228)
(1640,2.64163)
(1650,2.64092)
(1660,2.64017)
(1670,2.63946)
(1680,2.63873)
(1690,2.63806)
(1700,2.63731)
(1710,2.63661)
(1720,2.63593)
(1730,2.63528)
(1740,2.63461)
(1750,2.63395)
(1760,2.63326)
(1770,2.63265)
(1780,2.63198)
(1790,2.63128)
(1800,2.63062)
(1810,2.62993)
(1820,2.62932)
(1830,2.62866)
(1840,2.628)
(1850,2.62741)
(1860,2.62679)
(1870,2.62622)
(1880,2.62564)
(1890,2.62502)
(1900,2.62442)
(1910,2.62377)
(1920,2.62316)
(1930,2.62257)
(1940,2.62204)
(1950,2.62145)
(1960,2.62088)
(1970,2.62027)
(1980,2.61965)
(1990,2.61905)
(2000,2.61852)
(2010,2.61796)
(2020,2.61741)
(2030,2.61683)
(2040,2.61621)
(2050,2.61557)
(2060,2.61495)
(2070,2.61432)
(2080,2.6138)
(2090,2.61327)
(2100,2.61277)
(2110,2.61232)
(2120,2.61184)
(2130,2.61141)
(2140,2.61089)
(2150,2.6104)
(2160,2.60999)
(2170,2.60962)
(2180,2.60923)
(2190,2.60887)
(2200,2.60846)
(2210,2.6081)
(2220,2.60773)
(2230,2.60738)
(2240,2.60695)
(2250,2.60658)
(2260,2.60612)
(2270,2.60564)
(2280,2.60522)
(2290,2.60475)
(2300,2.60425)
(2310,2.60384)
(2320,2.60332)
(2330,2.60283)
(2340,2.60236)
(2350,2.6019)
(2360,2.60141)
(2370,2.60097)
(2380,2.60058)
(2390,2.60015)
(2400,2.59971)
(2410,2.5993)
(2420,2.59887)
(2430,2.59843)
(2440,2.59798)
(2450,2.59752)
(2460,2.59711)
(2470,2.59667)
(2480,2.59623)
(2490,2.59577)
(2500,2.59526)};\label{plots:plot3}

==> charts/minimization_NORB.tex <==
\addplot[black] coordinates{(0,6.53913)
(10,6.53913)
(20,6.53913)
(30,6.53913)
(40,6.53913)
(50,6.53913)
(60,6.53913)
(70,6.53913)
(80,6.53912)
(90,6.53879)
(100,6.5212)
(110,6.17897)
(120,5.75944)
(130,5.52096)
(140,5.35545)
(150,5.23206)
(160,5.13964)
(170,5.06601)
(180,4.99951)
(190,4.94361)
(200,4.89832)
(210,4.86127)
(220,4.83048)
(230,4.8042)
(240,4.78156)
(250,4.7514)
(260,4.44769)
(270,4.18893)
(280,4.00583)
(290,3.86288)
(300,3.74254)
(310,3.63637)
(320,3.54033)
(330,3.45277)
(340,3.37204)
(350,3.2976)
(360,3.2286)
(370,3.16446)
(380,3.10443)
(390,3.04795)
(400,2.99477)
(410,2.94449)
(420,2.8969)
(430,2.8518)
(440,2.80902)
(450,2.76812)
(460,2.72928)
(470,2.6922)
(480,2.65681)
(490,2.62287)
(500,2.59026)
(510,2.55887)
(520,2.52874)
(530,2.4999)
(540,2.47201)
(550,2.44509)
(560,2.41921)
(570,2.39428)
(580,2.37031)
(590,2.34717)
(600,2.32482)
(610,2.30314)
(620,2.28225)
(630,2.26185)
(640,2.24219)
(650,2.22294)
(660,2.20442)
(670,2.18631)
(680,2.16868)
(690,2.15164)
(700,2.13503)
(710,2.11893)
(720,2.1032)
(730,2.08795)
(740,2.07305)
(750,2.05849)
(760,2.04433)
(770,2.0306)
(780,2.01716)
(790,2.00409)
(800,1.99123)
(810,1.97869)
(820,1.96651)
(830,1.95456)
(840,1.94291)
(850,1.93145)
(860,1.92034)
(870,1.90942)
(880,1.89874)
(890,1.88834)
(900,1.87808)
(910,1.86805)
(920,1.85817)
(930,1.84854)
(940,1.83909)
(950,1.82981)
(960,1.82063)
(970,1.81162)
(980,1.80278)
(990,1.79411)
(1000,1.78574)
(1010,1.77758)
(1020,1.76957)
(1030,1.76168)
(1040,1.754)
(1050,1.74645)
(1060,1.73906)
(1070,1.73182)
(1080,1.72475)
(1090,1.71772)
(1100,1.71095)
(1110,1.70425)
(1120,1.69773)
(1130,1.69144)
(1140,1.6852)
(1150,1.6791)
(1160,1.67315)
(1170,1.66739)
(1180,1.66176)
(1190,1.65611)
(1200,1.65058)
(1210,1.64531)
(1220,1.6401)
(1230,1.63512)
(1240,1.6302)
(1250,1.62543)
(1260,1.62083)
(1270,1.61632)
(1280,1.61189)
(1290,1.60747)
(1300,1.60328)
(1310,1.59915)
(1320,1.59522)
(1330,1.59149)
(1340,1.58785)
(1350,1.58425)
(1360,1.58082)
(1370,1.57747)
(1380,1.57433)
(1390,1.57125)
(1400,1.56827)
(1410,1.56552)
(1420,1.56265)
(1430,1.55992)
(1440,1.55727)
(1450,1.55475)
(1460,1.5523)
(1470,1.55005)
(1480,1.54784)
(1490,1.54569)
(1500,1.5435)
(1510,1.5416)
(1520,1.53978)
(1530,1.53798)
(1540,1.53625)
(1550,1.53439)
(1560,1.53275)
(1570,1.531)
(1580,1.52916)
(1590,1.52744)
(1600,1.52572)
(1610,1.52423)
(1620,1.52285)
(1630,1.52154)
(1640,1.52013)
(1650,1.51882)
(1660,1.51755)
(1670,1.51642)
(1680,1.51519)
(1690,1.51404)
(1700,1.51288)
(1710,1.51175)
(1720,1.51066)
(1730,1.50951)
(1740,1.50825)
(1750,1.50709)
(1760,1.50594)
(1770,1.50475)
(1780,1.50357)
(1790,1.50242)
(1800,1.50122)
(1810,1.50006)
(1820,1.49887)
(1830,1.49769)
(1840,1.49656)
(1850,1.4954)
(1860,1.49425)
(1870,1.49308)
(1880,1.49197)
(1890,1.49084)
(1900,1.48976)
(1910,1.4886)
(1920,1.48752)
(1930,1.48639)
(1940,1.48526)
(1950,1.48414)
(1960,1.48299)
(1970,1.48187)
(1980,1.48077)
(1990,1.47957)
(2000,1.47837)
(2010,1.47719)
(2020,1.47609)
(2030,1.4749)
(2040,1.47378)
(2050,1.47261)
(2060,1.47146)
(2070,1.47039)
(2080,1.46933)
(2090,1.46823)
(2100,1.46712)
(2110,1.46603)
(2120,1.46491)
(2130,1.46384)
(2140,1.46272)
(2150,1.46163)
(2160,1.4605)
(2170,1.45942)
(2180,1.45831)
(2190,1.4572)
(2200,1.45613)
(2210,1.45498)
(2220,1.45381)
(2230,1.45269)
(2240,1.45158)
(2250,1.45044)
(2260,1.44937)
(2270,1.44827)
(2280,1.44724)
(2290,1.44619)
(2300,1.44509)
(2310,1.44403)
(2320,1.44296)
(2330,1.4419)
(2340,1.44075)
(2350,1.43973)
(2360,1.43869)
(2370,1.43761)
(2380,1.43652)
(2390,1.43543)
(2400,1.43434)
(2410,1.43334)
(2420,1.43231)
(2430,1.43132)
(2440,1.43036)
(2450,1.42933)
(2460,1.42823)
(2470,1.42721)
(2480,1.42619)
(2490,1.42517)
(2500,1.42422)};\label{plots:plot4}
\addplot[red] coordinates{(0,6.53913)
(10,6.53913)
(20,6.53913)
(30,6.53913)
(40,6.53913)
(50,6.53913)
(60,6.53913)
(70,6.53913)
(80,6.53912)
(90,6.53897)
(100,6.531)
(110,6.30321)
(120,5.91277)
(130,5.70326)
(140,5.53432)
(150,5.40716)
(160,5.32186)
(170,5.26166)
(180,5.21822)
(190,5.18601)
(200,5.16038)
(210,5.13973)
(220,5.1224)
(230,5.10748)
(240,5.09359)
(250,5.06648)
(260,4.66414)
(270,4.37053)
(280,4.18024)
(290,4.02481)
(300,3.88947)
(310,3.77009)
(320,3.66389)
(330,3.5686)
(340,3.48377)
(350,3.40523)
(360,3.33271)
(370,3.265)
(380,3.20187)
(390,3.14291)
(400,3.08765)
(410,3.03584)
(420,2.98704)
(430,2.94097)
(440,2.89725)
(450,2.85541)
(460,2.81559)
(470,2.77741)
(480,2.74086)
(490,2.70597)
(500,2.67245)
(510,2.6403)
(520,2.60959)
(530,2.58005)
(540,2.55162)
(550,2.52416)
(560,2.49762)
(570,2.47216)
(580,2.44751)
(590,2.42388)
(600,2.40103)
(610,2.37891)
(620,2.35744)
(630,2.33663)
(640,2.31649)
(650,2.29692)
(660,2.27784)
(670,2.2592)
(680,2.24119)
(690,2.22376)
(700,2.20697)
(710,2.1905)
(720,2.17455)
(730,2.15906)
(740,2.14403)
(750,2.12929)
(760,2.11494)
(770,2.10099)
(780,2.08724)
(790,2.07383)
(800,2.06084)
(810,2.04807)
(820,2.03564)
(830,2.02349)
(840,2.01154)
(850,1.99987)
(860,1.9885)
(870,1.97737)
(880,1.96645)
(890,1.95584)
(900,1.94546)
(910,1.93538)
(920,1.92552)
(930,1.91572)
(940,1.90622)
(950,1.89692)
(960,1.88784)
(970,1.879)
(980,1.87032)
(990,1.86178)
(1000,1.85355)
(1010,1.84536)
(1020,1.83746)
(1030,1.82961)
(1040,1.82194)
(1050,1.81456)
(1060,1.80729)
(1070,1.8002)
(1080,1.79323)
(1090,1.7866)
(1100,1.78003)
(1110,1.77354)
(1120,1.76713)
(1130,1.76088)
(1140,1.75487)
(1150,1.74903)
(1160,1.74338)
(1170,1.73777)
(1180,1.73224)
(1190,1.72694)
(1200,1.72167)
(1210,1.71648)
(1220,1.71148)
(1230,1.70664)
(1240,1.70187)
(1250,1.69715)
(1260,1.69256)
(1270,1.68822)
(1280,1.68407)
(1290,1.67998)
(1300,1.67606)
(1310,1.67217)
(1320,1.66846)
(1330,1.66489)
(1340,1.66132)
(1350,1.65776)
(1360,1.65445)
(1370,1.65112)
(1380,1.64794)
(1390,1.64496)
(1400,1.64188)
(1410,1.63888)
(1420,1.63604)
(1430,1.63338)
(1440,1.63082)
(1450,1.62827)
(1460,1.6259)
(1470,1.62351)
(1480,1.62126)
(1490,1.61908)
(1500,1.61689)
(1510,1.61479)
(1520,1.61271)
(1530,1.61061)
(1540,1.60874)
(1550,1.60684)
(1560,1.60501)
(1570,1.60333)
(1580,1.60162)
(1590,1.59985)
(1600,1.59815)
(1610,1.59655)
(1620,1.59499)
(1630,1.59339)
(1640,1.59182)
(1650,1.59031)
(1660,1.58887)
(1670,1.58737)
(1680,1.58594)
(1690,1.58453)
(1700,1.58313)
(1710,1.58173)
(1720,1.58037)
(1730,1.57903)
(1740,1.57763)
(1750,1.57625)
(1760,1.57489)
(1770,1.57356)
(1780,1.57223)
(1790,1.57089)
(1800,1.56961)
(1810,1.5683)
(1820,1.56699)
(1830,1.56565)
(1840,1.56434)
(1850,1.56298)
(1860,1.56162)
(1870,1.56029)
(1880,1.55896)
(1890,1.55758)
(1900,1.55619)
(1910,1.55489)
(1920,1.55361)
(1930,1.55225)
(1940,1.55091)
(1950,1.54963)
(1960,1.5484)
(1970,1.54715)
(1980,1.54594)
(1990,1.54469)
(2000,1.54344)
(2010,1.54218)
(2020,1.54095)
(2030,1.53972)
(2040,1.53856)
(2050,1.53742)
(2060,1.53625)
(2070,1.53514)
(2080,1.53408)
(2090,1.53303)
(2100,1.53197)
(2110,1.53087)
(2120,1.52983)
(2130,1.52876)
(2140,1.5277)
(2150,1.5266)
(2160,1.5255)
(2170,1.52446)
(2180,1.52341)
(2190,1.52232)
(2200,1.52131)
(2210,1.52028)
(2220,1.5192)
(2230,1.51816)
(2240,1.51711)
(2250,1.51612)
(2260,1.51508)
(2270,1.5142)
(2280,1.51322)
(2290,1.51225)
(2300,1.51131)
(2310,1.51034)
(2320,1.50941)
(2330,1.50836)
(2340,1.50735)
(2350,1.50634)
(2360,1.5053)
(2370,1.5043)
(2380,1.50336)
(2390,1.5024)
(2400,1.5014)
(2410,1.50043)
(2420,1.49951)
(2430,1.49863)
(2440,1.49775)
(2450,1.49692)
(2460,1.49609)
(2470,1.49528)
(2480,1.49453)
(2490,1.49378)
(2500,1.49306)};\label{plots:plot1}
\addplot[green] coordinates{(0,6.53913)
(10,6.53913)
(20,6.53913)
(30,6.53913)
(40,6.53913)
(50,6.53913)
(60,6.53913)
(70,6.53913)
(80,6.53912)
(90,6.53905)
(100,6.5347)
(110,6.39707)
(120,6.07085)
(130,5.8635)
(140,5.72467)
(150,5.61895)
(160,5.54625)
(170,5.49735)
(180,5.46121)
(190,5.43542)
(200,5.41779)
(210,5.40485)
(220,5.39456)
(230,5.38593)
(240,5.37848)
(250,5.35538)
(260,4.93351)
(270,4.59565)
(280,4.32489)
(290,4.14362)
(300,4.00001)
(310,3.88041)
(320,3.77559)
(330,3.68164)
(340,3.59669)
(350,3.51892)
(360,3.44662)
(370,3.37933)
(380,3.31655)
(390,3.2578)
(400,3.20246)
(410,3.15001)
(420,3.10052)
(430,3.05365)
(440,3.00914)
(450,2.9667)
(460,2.92641)
(470,2.8881)
(480,2.85164)
(490,2.81657)
(500,2.78279)
(510,2.75049)
(520,2.71961)
(530,2.68994)
(540,2.66143)
(550,2.63398)
(560,2.60745)
(570,2.58194)
(580,2.55741)
(590,2.53368)
(600,2.51064)
(610,2.48838)
(620,2.46698)
(630,2.44618)
(640,2.42587)
(650,2.40606)
(660,2.38687)
(670,2.36826)
(680,2.35022)
(690,2.33276)
(700,2.31581)
(710,2.29937)
(720,2.28339)
(730,2.26785)
(740,2.25277)
(750,2.23798)
(760,2.22355)
(770,2.20937)
(780,2.19561)
(790,2.18214)
(800,2.16898)
(810,2.15613)
(820,2.14345)
(830,2.13106)
(840,2.11899)
(850,2.10711)
(860,2.09552)
(870,2.08414)
(880,2.07297)
(890,2.06223)
(900,2.05178)
(910,2.04165)
(920,2.03167)
(930,2.02213)
(940,2.01257)
(950,2.00311)
(960,1.99387)
(970,1.98483)
(980,1.97604)
(990,1.96743)
(1000,1.95923)
(1010,1.95108)
(1020,1.94326)
(1030,1.93548)
(1040,1.92783)
(1050,1.92038)
(1060,1.91306)
(1070,1.90589)
(1080,1.89891)
(1090,1.89196)
(1100,1.88528)
(1110,1.87883)
(1120,1.87251)
(1130,1.86642)
(1140,1.86035)
(1150,1.85447)
(1160,1.84877)
(1170,1.8431)
(1180,1.8378)
(1190,1.83256)
(1200,1.82749)
(1210,1.82264)
(1220,1.818)
(1230,1.8134)
(1240,1.809)
(1250,1.80472)
(1260,1.80054)
(1270,1.79661)
(1280,1.79269)
(1290,1.78895)
(1300,1.78543)
(1310,1.78201)
(1320,1.77854)
(1330,1.7752)
(1340,1.77195)
(1350,1.76898)
(1360,1.76611)
(1370,1.76336)
(1380,1.76089)
(1390,1.75836)
(1400,1.75598)
(1410,1.75372)
(1420,1.75162)
(1430,1.74956)
(1440,1.74756)
(1450,1.74566)
(1460,1.74382)
(1470,1.74207)
(1480,1.7403)
(1490,1.73875)
(1500,1.73749)
(1510,1.73612)
(1520,1.73487)
(1530,1.73367)
(1540,1.73257)
(1550,1.73155)
(1560,1.7306)
(1570,1.7296)
(1580,1.72864)
(1590,1.72775)
(1600,1.72692)
(1610,1.72611)
(1620,1.72539)
(1630,1.72457)
(1640,1.72377)
(1650,1.72291)
(1660,1.72206)
(1670,1.72124)
(1680,1.72039)
(1690,1.71955)
(1700,1.71868)
(1710,1.71779)
(1720,1.71692)
(1730,1.71618)
(1740,1.71526)
(1750,1.71436)
(1760,1.71349)
(1770,1.71251)
(1780,1.71144)
(1790,1.71047)
(1800,1.70951)
(1810,1.70854)
(1820,1.70764)
(1830,1.70665)
(1840,1.70561)
(1850,1.70464)
(1860,1.70368)
(1870,1.70268)
(1880,1.70165)
(1890,1.70062)
(1900,1.69959)
(1910,1.69856)
(1920,1.6975)
(1930,1.69643)
(1940,1.69545)
(1950,1.69437)
(1960,1.69325)
(1970,1.69211)
(1980,1.69097)
(1990,1.68984)
(2000,1.68872)
(2010,1.6876)
(2020,1.68649)
(2030,1.68528)
(2040,1.68415)
(2050,1.68296)
(2060,1.68184)
(2070,1.68075)
(2080,1.67967)
(2090,1.67854)
(2100,1.67747)
(2110,1.6764)
(2120,1.67524)
(2130,1.67411)
(2140,1.67301)
(2150,1.67195)
(2160,1.67087)
(2170,1.66984)
(2180,1.66881)
(2190,1.66783)
(2200,1.66689)
(2210,1.66592)
(2220,1.66497)
(2230,1.66394)
(2240,1.66292)
(2250,1.66193)
(2260,1.66092)
(2270,1.65991)
(2280,1.6589)
(2290,1.65799)
(2300,1.65702)
(2310,1.6561)
(2320,1.6552)
(2330,1.65425)
(2340,1.65341)
(2350,1.65251)
(2360,1.65158)
(2370,1.6508)
(2380,1.64999)
(2390,1.64918)
(2400,1.64836)
(2410,1.64753)
(2420,1.64666)
(2430,1.64582)
(2440,1.64497)
(2450,1.6441)
(2460,1.64337)
(2470,1.64261)
(2480,1.64183)
(2490,1.64105)
(2500,1.64037)};\label{plots:plot2}
\addplot[blue] coordinates{(0,6.53913)
(10,6.53913)
(20,6.53913)
(30,6.53913)
(40,6.53913)
(50,6.53913)
(60,6.53913)
(70,6.53913)
(80,6.53913)
(90,6.53912)
(100,6.53881)
(110,6.52504)
(120,6.38336)
(130,6.25637)
(140,6.17167)
(150,6.13739)
(160,6.12307)
(170,6.11557)
(180,6.11069)
(190,6.10682)
(200,6.10439)
(210,6.10263)
(220,6.10155)
(230,6.10085)
(240,6.10044)
(250,6.08217)
(260,5.69493)
(270,5.44155)
(280,5.22735)
(290,4.98581)
(300,4.77145)
(310,4.59679)
(320,4.45045)
(330,4.32572)
(340,4.21841)
(350,4.12379)
(360,4.03968)
(370,3.96293)
(380,3.89249)
(390,3.82785)
(400,3.76823)
(410,3.71256)
(420,3.66034)
(430,3.61147)
(440,3.56536)
(450,3.52141)
(460,3.4802)
(470,3.44159)
(480,3.40487)
(490,3.37007)
(500,3.33692)
(510,3.30535)
(520,3.27506)
(530,3.24582)
(540,3.21815)
(550,3.19184)
(560,3.16657)
(570,3.14224)
(580,3.11867)
(590,3.09608)
(600,3.07425)
(610,3.05334)
(620,3.03313)
(630,3.01368)
(640,2.99488)
(650,2.97667)
(660,2.95894)
(670,2.94162)
(680,2.92465)
(690,2.90811)
(700,2.89198)
(710,2.87624)
(720,2.86101)
(730,2.84635)
(740,2.83204)
(750,2.8181)
(760,2.80452)
(770,2.79119)
(780,2.77833)
(790,2.76577)
(800,2.75361)
(810,2.74177)
(820,2.73038)
(830,2.7192)
(840,2.70816)
(850,2.69738)
(860,2.68692)
(870,2.67669)
(880,2.66672)
(890,2.65697)
(900,2.64741)
(910,2.63804)
(920,2.62885)
(930,2.61991)
(940,2.61115)
(950,2.60258)
(960,2.5942)
(970,2.58589)
(980,2.57774)
(990,2.56971)
(1000,2.56184)
(1010,2.55407)
(1020,2.54652)
(1030,2.53926)
(1040,2.53219)
(1050,2.52538)
(1060,2.51872)
(1070,2.51219)
(1080,2.50577)
(1090,2.49954)
(1100,2.49339)
(1110,2.48733)
(1120,2.4815)
(1130,2.47579)
(1140,2.47026)
(1150,2.46478)
(1160,2.45953)
(1170,2.45432)
(1180,2.44918)
(1190,2.44415)
(1200,2.4392)
(1210,2.43441)
(1220,2.42966)
(1230,2.42502)
(1240,2.42047)
(1250,2.41603)
(1260,2.41168)
(1270,2.40752)
(1280,2.40338)
(1290,2.39954)
(1300,2.39586)
(1310,2.39234)
(1320,2.38899)
(1330,2.38567)
(1340,2.38253)
(1350,2.37975)
(1360,2.37714)
(1370,2.37452)
(1380,2.37197)
(1390,2.3697)
(1400,2.3675)
(1410,2.36534)
(1420,2.36326)
(1430,2.36131)
(1440,2.35945)
(1450,2.35774)
(1460,2.35608)
(1470,2.35439)
(1480,2.35281)
(1490,2.35122)
(1500,2.34972)
(1510,2.3483)
(1520,2.3469)
(1530,2.34554)
(1540,2.34432)
(1550,2.34304)
(1560,2.34176)
(1570,2.34045)
(1580,2.33927)
(1590,2.33803)
(1600,2.33686)
(1610,2.33567)
(1620,2.33445)
(1630,2.33324)
(1640,2.33205)
(1650,2.33086)
(1660,2.32974)
(1670,2.32855)
(1680,2.32737)
(1690,2.32624)
(1700,2.32508)
(1710,2.32396)
(1720,2.32287)
(1730,2.32184)
(1740,2.32065)
(1750,2.31943)
(1760,2.3182)
(1770,2.31702)
(1780,2.31586)
(1790,2.31465)
(1800,2.31347)
(1810,2.31239)
(1820,2.31125)
(1830,2.31011)
(1840,2.30901)
(1850,2.30786)
(1860,2.30678)
(1870,2.30575)
(1880,2.30461)
(1890,2.30344)
(1900,2.30237)
(1910,2.30129)
(1920,2.3002)
(1930,2.29919)
(1940,2.29824)
(1950,2.29724)
(1960,2.29624)
(1970,2.29524)
(1980,2.29423)
(1990,2.29327)
(2000,2.29226)
(2010,2.29129)
(2020,2.29042)
(2030,2.28952)
(2040,2.28856)
(2050,2.28759)
(2060,2.28675)
(2070,2.28587)
(2080,2.28509)
(2090,2.28442)
(2100,2.28373)
(2110,2.28294)
(2120,2.28217)
(2130,2.28145)
(2140,2.28069)
(2150,2.27988)
(2160,2.27909)
(2170,2.27828)
(2180,2.27747)
(2190,2.27661)
(2200,2.27579)
(2210,2.27498)
(2220,2.27418)
(2230,2.27338)
(2240,2.27259)
(2250,2.27172)
(2260,2.27083)
(2270,2.26998)
(2280,2.26915)
(2290,2.26828)
(2300,2.26748)
(2310,2.2667)
(2320,2.26588)
(2330,2.26503)
(2340,2.26419)
(2350,2.26335)
(2360,2.26254)
(2370,2.26161)
(2380,2.26072)
(2390,2.2598)
(2400,2.25881)
(2410,2.25779)
(2420,2.25679)
(2430,2.25582)
(2440,2.25499)
(2450,2.25417)
(2460,2.25345)
(2470,2.25269)
(2480,2.2519)
(2490,2.25111)
(2500,2.25038)};\label{plots:plot3}

==> charts/minimization_TIMIT.tex <==

\addplot[black] coordinates{(0,7.19875)
(10,7.19875)
(20,7.19875)
(30,7.19875)
(40,7.19875)
(50,7.19875)
(60,7.19875)
(70,7.19875)
(80,7.19875)
(90,7.19875)
(100,7.19875)
(110,7.19874)
(120,7.19856)
(130,7.19592)
(140,7.18688)
(150,7.18124)
(160,7.17885)
(170,7.1775)
(180,7.17661)
(190,7.17588)
(200,7.17483)
(210,7.17146)
(220,7.15648)
(230,7.10683)
(240,7.0381)
(250,6.9824)
(260,6.56294)
(270,6.27938)
(280,6.08462)
(290,5.83868)
(300,5.60601)
(310,5.43878)
(320,5.31326)
(330,5.21296)
(340,5.12948)
(350,5.05786)
(360,4.99495)
(370,4.93859)
(380,4.88726)
(390,4.84026)
(400,4.79695)
(410,4.75668)
(420,4.71904)
(430,4.68358)
(440,4.65012)
(450,4.61842)
(460,4.5884)
(470,4.5598)
(480,4.53268)
(490,4.50674)
(500,4.48186)
(510,4.45801)
(520,4.43519)
(530,4.41315)
(540,4.392)
(550,4.37152)
(560,4.35167)
(570,4.33254)
(580,4.31407)
(590,4.29626)
(600,4.27901)
(610,4.26227)
(620,4.24604)
(630,4.23021)
(640,4.21486)
(650,4.19997)
(660,4.1855)
(670,4.17143)
(680,4.15776)
(690,4.14442)
(700,4.13141)
(710,4.11871)
(720,4.10629)
(730,4.09415)
(740,4.08233)
(750,4.07076)
(760,4.05942)
(770,4.04832)
(780,4.03743)
(790,4.02678)
(800,4.01637)
(810,4.00617)
(820,3.99617)
(830,3.98634)
(840,3.97669)
(850,3.96718)
(860,3.95782)
(870,3.94859)
(880,3.93955)
(890,3.93069)
(900,3.92204)
(910,3.91352)
(920,3.90517)
(930,3.8969)
(940,3.88878)
(950,3.88077)
(960,3.87296)
(970,3.86533)
(980,3.85778)
(990,3.85035)
(1000,3.84301)
(1010,3.83579)
(1020,3.82864)
(1030,3.82162)
(1040,3.81477)
(1050,3.80804)
(1060,3.80142)
(1070,3.79498)
(1080,3.78863)
(1090,3.78238)
(1100,3.77619)
(1110,3.77007)
(1120,3.76411)
(1130,3.75824)
(1140,3.75245)
(1150,3.7467)
(1160,3.74104)
(1170,3.73543)
(1180,3.72987)
(1190,3.72439)
(1200,3.71898)
(1210,3.71359)
(1220,3.70822)
(1230,3.70291)
(1240,3.69764)
(1250,3.69244)
(1260,3.68732)
(1270,3.68225)
(1280,3.67725)
(1290,3.67231)
(1300,3.66743)
(1310,3.66264)
(1320,3.6579)
(1330,3.65323)
(1340,3.64862)
(1350,3.64403)
(1360,3.63952)
(1370,3.63504)
(1380,3.63061)
(1390,3.62623)
(1400,3.62191)
(1410,3.61766)
(1420,3.61346)
(1430,3.60928)
(1440,3.60517)
(1450,3.60108)
(1460,3.59701)
(1470,3.59301)
(1480,3.58904)
(1490,3.5851)
(1500,3.58118)
(1510,3.57732)
(1520,3.57348)
(1530,3.56967)
(1540,3.5659)
(1550,3.5622)
(1560,3.55851)
(1570,3.55487)
(1580,3.55128)
(1590,3.54771)
(1600,3.5442)
(1610,3.5407)
(1620,3.53724)
(1630,3.53382)
(1640,3.53045)
(1650,3.52713)
(1660,3.52382)
(1670,3.52049)
(1680,3.51719)
(1690,3.51392)
(1700,3.51066)
(1710,3.50747)
(1720,3.5043)
(1730,3.50113)
(1740,3.49803)
(1750,3.49494)
(1760,3.49191)
(1770,3.48888)
(1780,3.4859)
(1790,3.4829)
(1800,3.48001)
(1810,3.47715)
(1820,3.47428)
(1830,3.47146)
(1840,3.46863)
(1850,3.46588)
(1860,3.46316)
(1870,3.46048)
(1880,3.45783)
(1890,3.45519)
(1900,3.45264)
(1910,3.4501)
(1920,3.44757)
(1930,3.44508)
(1940,3.44266)
(1950,3.44028)
(1960,3.43796)
(1970,3.43562)
(1980,3.43334)
(1990,3.4311)
(2000,3.42892)
(2010,3.42678)
(2020,3.42468)
(2030,3.42255)
(2040,3.42053)
(2050,3.41852)
(2060,3.41663)
(2070,3.4147)
(2080,3.41293)
(2090,3.41117)
(2100,3.40944)
(2110,3.40777)
(2120,3.40615)
(2130,3.4047)
(2140,3.40321)
(2150,3.4018)
(2160,3.40049)
(2170,3.39921)
(2180,3.39804)
(2190,3.3968)
(2200,3.39573)
(2210,3.39466)
(2220,3.39364)
(2230,3.39268)
(2240,3.39173)
(2250,3.39082)
(2260,3.38995)
(2270,3.38915)
(2280,3.38832)
(2290,3.38752)
(2300,3.38675)
(2310,3.38598)
(2320,3.38526)
(2330,3.38455)
(2340,3.38388)
(2350,3.38312)
(2360,3.38247)
(2370,3.38185)
(2380,3.38119)
(2390,3.38058)
(2400,3.38002)
(2410,3.37949)
(2420,3.37895)
(2430,3.37842)
(2440,3.37786)
(2450,3.3774)
(2460,3.37689)
(2470,3.37644)
(2480,3.376)
(2490,3.37565)
(2500,3.37526)};\label{plots:plot4}
\addplot[red] coordinates{(0,7.19875)
(10,7.19875)
(20,7.19875)
(30,7.19875)
(40,7.19875)
(50,7.19875)
(60,7.19875)
(70,7.19875)
(80,7.19875)
(90,7.19875)
(100,7.19875)
(110,7.19874)
(120,7.19856)
(130,7.19595)
(140,7.18694)
(150,7.1813)
(160,7.17889)
(170,7.17753)
(180,7.17661)
(190,7.17575)
(200,7.17411)
(210,7.16805)
(220,7.14354)
(230,7.08505)
(240,7.02875)
(250,6.98496)
(260,6.56337)
(270,6.26971)
(280,5.99528)
(290,5.7188)
(300,5.52282)
(310,5.37606)
(320,5.26004)
(330,5.16451)
(340,5.08337)
(350,5.01261)
(360,4.9496)
(370,4.89272)
(380,4.84078)
(390,4.79305)
(400,4.74886)
(410,4.7077)
(420,4.66915)
(430,4.63297)
(440,4.59907)
(450,4.56696)
(460,4.53653)
(470,4.5077)
(480,4.48035)
(490,4.45431)
(500,4.42942)
(510,4.40568)
(520,4.38292)
(530,4.36107)
(540,4.3401)
(550,4.31989)
(560,4.30039)
(570,4.28165)
(580,4.26348)
(590,4.24594)
(600,4.22896)
(610,4.21255)
(620,4.19664)
(630,4.18117)
(640,4.16614)
(650,4.15155)
(660,4.13732)
(670,4.12345)
(680,4.10993)
(690,4.09674)
(700,4.08386)
(710,4.07129)
(720,4.05903)
(730,4.04709)
(740,4.03542)
(750,4.02403)
(760,4.01291)
(770,4.00205)
(780,3.99142)
(790,3.98103)
(800,3.97083)
(810,3.96083)
(820,3.95101)
(830,3.94144)
(840,3.93207)
(850,3.9229)
(860,3.9139)
(870,3.90504)
(880,3.89631)
(890,3.88773)
(900,3.87931)
(910,3.87106)
(920,3.86294)
(930,3.85496)
(940,3.84704)
(950,3.83905)
(960,3.83117)
(970,3.82341)
(980,3.81582)
(990,3.80842)
(1000,3.80113)
(1010,3.79404)
(1020,3.78709)
(1030,3.78028)
(1040,3.7736)
(1050,3.76703)
(1060,3.76048)
(1070,3.75404)
(1080,3.74791)
(1090,3.7422)
(1100,3.73671)
(1110,3.73132)
(1120,3.72596)
(1130,3.72014)
(1140,3.71445)
(1150,3.70882)
(1160,3.70324)
(1170,3.6977)
(1180,3.69224)
(1190,3.68687)
(1200,3.68156)
(1210,3.67632)
(1220,3.67117)
(1230,3.66607)
(1240,3.661)
(1250,3.65599)
(1260,3.65103)
(1270,3.64613)
(1280,3.64128)
(1290,3.63651)
(1300,3.63177)
(1310,3.62709)
(1320,3.62251)
(1330,3.61796)
(1340,3.61343)
(1350,3.60894)
(1360,3.60452)
(1370,3.60015)
(1380,3.59583)
(1390,3.59154)
(1400,3.58728)
(1410,3.58309)
(1420,3.57893)
(1430,3.5748)
(1440,3.57072)
(1450,3.56673)
(1460,3.56275)
(1470,3.55884)
(1480,3.55495)
(1490,3.55108)
(1500,3.54724)
(1510,3.54343)
(1520,3.53967)
(1530,3.53593)
(1540,3.53226)
(1550,3.52859)
(1560,3.525)
(1570,3.52143)
(1580,3.51788)
(1590,3.51437)
(1600,3.5109)
(1610,3.50748)
(1620,3.50411)
(1630,3.50073)
(1640,3.4974)
(1650,3.49409)
(1660,3.49079)
(1670,3.48753)
(1680,3.48434)
(1690,3.48116)
(1700,3.47803)
(1710,3.47497)
(1720,3.47189)
(1730,3.46884)
(1740,3.46584)
(1750,3.46286)
(1760,3.45989)
(1770,3.45698)
(1780,3.45411)
(1790,3.45128)
(1800,3.44843)
(1810,3.44564)
(1820,3.44286)
(1830,3.4401)
(1840,3.43737)
(1850,3.43468)
(1860,3.43201)
(1870,3.42942)
(1880,3.4268)
(1890,3.42422)
(1900,3.42172)
(1910,3.41923)
(1920,3.41673)
(1930,3.41428)
(1940,3.41183)
(1950,3.40942)
(1960,3.40703)
(1970,3.40465)
(1980,3.40231)
(1990,3.39998)
(2000,3.39769)
(2010,3.39546)
(2020,3.39325)
(2030,3.39108)
(2040,3.38894)
(2050,3.38685)
(2060,3.38475)
(2070,3.38272)
(2080,3.38071)
(2090,3.37875)
(2100,3.37681)
(2110,3.37487)
(2120,3.37297)
(2130,3.37107)
(2140,3.36923)
(2150,3.3674)
(2160,3.36562)
(2170,3.36391)
(2180,3.3622)
(2190,3.36054)
(2200,3.3589)
(2210,3.35729)
(2220,3.35575)
(2230,3.35423)
(2240,3.35272)
(2250,3.35123)
(2260,3.34979)
(2270,3.34841)
(2280,3.347)
(2290,3.34568)
(2300,3.34444)
(2310,3.34318)
(2320,3.34205)
(2330,3.34097)
(2340,3.33989)
(2350,3.33888)
(2360,3.33795)
(2370,3.33709)
(2380,3.33625)
(2390,3.33554)
(2400,3.33481)
(2410,3.33417)
(2420,3.33355)
(2430,3.33298)
(2440,3.33249)
(2450,3.33202)
(2460,3.33157)
(2470,3.33121)
(2480,3.33085)
(2490,3.33054)
(2500,3.33026)};\label{plots:plot1}
\addplot[green] coordinates{(0,7.19875)
(10,7.19875)
(20,7.19875)
(30,7.19875)
(40,7.19875)
(50,7.19875)
(60,7.19875)
(70,7.19875)
(80,7.19875)
(90,7.19875)
(100,7.19875)
(110,7.19874)
(120,7.19858)
(130,7.19614)
(140,7.18733)
(150,7.18151)
(160,7.17901)
(170,7.17761)
(180,7.17663)
(190,7.17562)
(200,7.17349)
(210,7.16599)
(220,7.14005)
(230,7.08849)
(240,7.04306)
(250,7.00529)
(260,6.57575)
(270,6.27662)
(280,6.00574)
(290,5.73172)
(300,5.53371)
(310,5.38395)
(320,5.26582)
(330,5.16942)
(340,5.08801)
(350,5.01725)
(360,4.95454)
(370,4.89803)
(380,4.84659)
(390,4.79918)
(400,4.75527)
(410,4.71441)
(420,4.67623)
(430,4.6404)
(440,4.6067)
(450,4.57487)
(460,4.54477)
(470,4.51628)
(480,4.48941)
(490,4.46366)
(500,4.43913)
(510,4.41565)
(520,4.39313)
(530,4.37159)
(540,4.35085)
(550,4.3309)
(560,4.31171)
(570,4.29319)
(580,4.27525)
(590,4.25784)
(600,4.241)
(610,4.22473)
(620,4.20901)
(630,4.19379)
(640,4.17901)
(650,4.16464)
(660,4.15061)
(670,4.13697)
(680,4.12368)
(690,4.11073)
(700,4.09814)
(710,4.08585)
(720,4.0739)
(730,4.06219)
(740,4.05077)
(750,4.03965)
(760,4.02875)
(770,4.01808)
(780,4.00764)
(790,3.99743)
(800,3.98742)
(810,3.97756)
(820,3.9679)
(830,3.95845)
(840,3.94916)
(850,3.94009)
(860,3.93115)
(870,3.92239)
(880,3.91377)
(890,3.90531)
(900,3.89698)
(910,3.88883)
(920,3.8808)
(930,3.87291)
(940,3.86515)
(950,3.85754)
(960,3.85008)
(970,3.84275)
(980,3.83554)
(990,3.82845)
(1000,3.82142)
(1010,3.81448)
(1020,3.80767)
(1030,3.80093)
(1040,3.79432)
(1050,3.78778)
(1060,3.78136)
(1070,3.77507)
(1080,3.76889)
(1090,3.76278)
(1100,3.75671)
(1110,3.75075)
(1120,3.74476)
(1130,3.73882)
(1140,3.73307)
(1150,3.72738)
(1160,3.72178)
(1170,3.71626)
(1180,3.71086)
(1190,3.70552)
(1200,3.70029)
(1210,3.69509)
(1220,3.68996)
(1230,3.68488)
(1240,3.67987)
(1250,3.67491)
(1260,3.67002)
(1270,3.66519)
(1280,3.66041)
(1290,3.6556)
(1300,3.6509)
(1310,3.64629)
(1320,3.64172)
(1330,3.6372)
(1340,3.63272)
(1350,3.62827)
(1360,3.62387)
(1370,3.6195)
(1380,3.6152)
(1390,3.61094)
(1400,3.60677)
(1410,3.60265)
(1420,3.59855)
(1430,3.59446)
(1440,3.59044)
(1450,3.58649)
(1460,3.58263)
(1470,3.57877)
(1480,3.57497)
(1490,3.57123)
(1500,3.56752)
(1510,3.56387)
(1520,3.56018)
(1530,3.55654)
(1540,3.55294)
(1550,3.54938)
(1560,3.54587)
(1570,3.54239)
(1580,3.53899)
(1590,3.53564)
(1600,3.53232)
(1610,3.52902)
(1620,3.52576)
(1630,3.52253)
(1640,3.51933)
(1650,3.51615)
(1660,3.51303)
(1670,3.50994)
(1680,3.5069)
(1690,3.50387)
(1700,3.50088)
(1710,3.49791)
(1720,3.49499)
(1730,3.49206)
(1740,3.48921)
(1750,3.48641)
(1760,3.48364)
(1770,3.48095)
(1780,3.47829)
(1790,3.47566)
(1800,3.47307)
(1810,3.47047)
(1820,3.46796)
(1830,3.46548)
(1840,3.46305)
(1850,3.46064)
(1860,3.45827)
(1870,3.45592)
(1880,3.45358)
(1890,3.45134)
(1900,3.4491)
(1910,3.4469)
(1920,3.44476)
(1930,3.44268)
(1940,3.44063)
(1950,3.43863)
(1960,3.43668)
(1970,3.43475)
(1980,3.43289)
(1990,3.43104)
(2000,3.42921)
(2010,3.42738)
(2020,3.42562)
(2030,3.42389)
(2040,3.42219)
(2050,3.42051)
(2060,3.41884)
(2070,3.4172)
(2080,3.4156)
(2090,3.41403)
(2100,3.41247)
(2110,3.41096)
(2120,3.40943)
(2130,3.40797)
(2140,3.40656)
(2150,3.40514)
(2160,3.40377)
(2170,3.40243)
(2180,3.40115)
(2190,3.39985)
(2200,3.39858)
(2210,3.39736)
(2220,3.39616)
(2230,3.39497)
(2240,3.3938)
(2250,3.3926)
(2260,3.39147)
(2270,3.39037)
(2280,3.38928)
(2290,3.38822)
(2300,3.38718)
(2310,3.38619)
(2320,3.38515)
(2330,3.38414)
(2340,3.38317)
(2350,3.3822)
(2360,3.38123)
(2370,3.38029)
(2380,3.37936)
(2390,3.37846)
(2400,3.37756)
(2410,3.37669)
(2420,3.37582)
(2430,3.375)
(2440,3.37421)
(2450,3.37341)
(2460,3.37261)
(2470,3.37189)
(2480,3.37115)
(2490,3.37042)
(2500,3.36977)};\label{plots:plot2}
\addplot[blue] coordinates{(0,7.19875)
(10,7.19875)
(20,7.19875)
(30,7.19875)
(40,7.19875)
(50,7.19875)
(60,7.19875)
(70,7.19875)
(80,7.19875)
(90,7.19875)
(100,7.19875)
(110,7.19875)
(120,7.19873)
(130,7.19854)
(140,7.19642)
(150,7.191)
(160,7.18546)
(170,7.18229)
(180,7.18073)
(190,7.17983)
(200,7.17925)
(210,7.17881)
(220,7.17847)
(230,7.17815)
(240,7.17782)
(250,7.17707)
(260,7.04807)
(270,6.5439)
(280,6.23956)
(290,5.9946)
(300,5.791)
(310,5.63957)
(320,5.52314)
(330,5.42943)
(340,5.35047)
(350,5.28172)
(360,5.22067)
(370,5.1654)
(380,5.11471)
(390,5.06792)
(400,5.02453)
(410,4.9842)
(420,4.94668)
(430,4.91151)
(440,4.87845)
(450,4.84736)
(460,4.81803)
(470,4.79033)
(480,4.76401)
(490,4.73893)
(500,4.71492)
(510,4.69195)
(520,4.67012)
(530,4.64935)
(540,4.62941)
(550,4.61025)
(560,4.59178)
(570,4.57406)
(580,4.55692)
(590,4.54038)
(600,4.52449)
(610,4.50919)
(620,4.49439)
(630,4.48009)
(640,4.46627)
(650,4.45289)
(660,4.43993)
(670,4.42735)
(680,4.41515)
(690,4.40328)
(700,4.39178)
(710,4.38058)
(720,4.36962)
(730,4.35895)
(740,4.34853)
(750,4.3384)
(760,4.32851)
(770,4.31882)
(780,4.30934)
(790,4.30003)
(800,4.29095)
(810,4.28209)
(820,4.2734)
(830,4.26489)
(840,4.25653)
(850,4.24829)
(860,4.24021)
(870,4.23228)
(880,4.22449)
(890,4.21685)
(900,4.20939)
(910,4.20205)
(920,4.19483)
(930,4.18774)
(940,4.18078)
(950,4.17393)
(960,4.16721)
(970,4.16059)
(980,4.15408)
(990,4.14762)
(1000,4.14127)
(1010,4.13506)
(1020,4.12892)
(1030,4.12289)
(1040,4.11694)
(1050,4.11108)
(1060,4.1053)
(1070,4.09963)
(1080,4.09403)
(1090,4.08854)
(1100,4.08316)
(1110,4.07782)
(1120,4.07256)
(1130,4.06735)
(1140,4.06221)
(1150,4.05711)
(1160,4.05211)
(1170,4.04716)
(1180,4.0423)
(1190,4.0375)
(1200,4.03273)
(1210,4.02805)
(1220,4.02346)
(1230,4.01897)
(1240,4.01451)
(1250,4.01011)
(1260,4.0058)
(1270,4.00152)
(1280,3.99731)
(1290,3.99318)
(1300,3.9891)
(1310,3.9851)
(1320,3.98112)
(1330,3.97719)
(1340,3.97331)
(1350,3.96948)
(1360,3.96567)
(1370,3.96194)
(1380,3.95823)
(1390,3.95452)
(1400,3.95088)
(1410,3.94733)
(1420,3.94379)
(1430,3.94031)
(1440,3.93688)
(1450,3.9335)
(1460,3.9302)
(1470,3.9269)
(1480,3.92363)
(1490,3.92039)
(1500,3.91721)
(1510,3.91401)
(1520,3.9109)
(1530,3.90785)
(1540,3.90483)
(1550,3.90184)
(1560,3.89888)
(1570,3.89593)
(1580,3.89303)
(1590,3.89016)
(1600,3.88732)
(1610,3.88446)
(1620,3.88162)
(1630,3.8788)
(1640,3.87606)
(1650,3.87336)
(1660,3.87068)
(1670,3.86802)
(1680,3.86538)
(1690,3.86271)
(1700,3.86007)
(1710,3.85749)
(1720,3.85492)
(1730,3.85236)
(1740,3.84983)
(1750,3.8473)
(1760,3.84479)
(1770,3.84229)
(1780,3.83984)
(1790,3.83743)
(1800,3.83507)
(1810,3.83266)
(1820,3.83031)
(1830,3.82798)
(1840,3.82567)
(1850,3.8234)
(1860,3.82118)
(1870,3.81897)
(1880,3.81675)
(1890,3.81459)
(1900,3.81244)
(1910,3.81028)
(1920,3.80814)
(1930,3.80606)
(1940,3.804)
(1950,3.80196)
(1960,3.79993)
(1970,3.79794)
(1980,3.79594)
(1990,3.79402)
(2000,3.79212)
(2010,3.79028)
(2020,3.78846)
(2030,3.78671)
(2040,3.78499)
(2050,3.78332)
(2060,3.7817)
(2070,3.78014)
(2080,3.7786)
(2090,3.77708)
(2100,3.7756)
(2110,3.77413)
(2120,3.77273)
(2130,3.77137)
(2140,3.77002)
(2150,3.76871)
(2160,3.76744)
(2170,3.76617)
(2180,3.7649)
(2190,3.7637)
(2200,3.76252)
(2210,3.76137)
(2220,3.76026)
(2230,3.75917)
(2240,3.75812)
(2250,3.75708)
(2260,3.75605)
(2270,3.75503)
(2280,3.75404)
(2290,3.75307)
(2300,3.75211)
(2310,3.75119)
(2320,3.7503)
(2330,3.74947)
(2340,3.74861)
(2350,3.74779)
(2360,3.74697)
(2370,3.74616)
(2380,3.74537)
(2390,3.74461)
(2400,3.74385)
(2410,3.74314)
(2420,3.74244)
(2430,3.74174)
(2440,3.7411)
(2450,3.74046)
(2460,3.73982)
(2470,3.73919)
(2480,3.73856)
(2490,3.73795)
(2500,3.73734)};\label{plots:plot3}

==> charts/precision_CIFAR.tex <==
\addplot[green] coordinates{
(100,1)
(150,1)
(200,1)
(250,1)
(300,1)
(400,1)
(500,1)
(1000,0.86)
(2000,0.688)
(3000,0.6)
(4000,0.55)
(5000,0.51)
(7500,0.46)
(10000,0.42)
(15000,0.39)
(20000,0.353)
(30000,0.326)
};\label{plots:plot2}
\addplot[red] coordinates{
(100,1)
(150,1)
(200,1)
(250,1)
(300,1)
(400,1)
(500,1)
(1000,1)
(2000,0.923)
(3000,0.849)
(4000,0.79)
(5000,0.74)
(7500,0.68)
(10000,0.64)
(15000,0.59)
(20000,0.554)
(30000,0.502)
};\label{plots:plot1}
\addplot[blue] coordinates{
(100,0.845)
(150,0.75)
(200,0.625)
(250,0.573)
(300,0.52)
(400,0.421)
(500,0.39)
(1000,0.273)
(2000,0.236)
(3000,0.202)
(4000,0.187)
(5000,0.18)
(7500,0.15)
(10000,0.13)
(15000,0.1218)
(20000,0.11)
(30000,0.1)
};\label{plots:plot3}
\addplot[black] coordinates{
(100,1)
(30000,1)
};\label{plots:plot4}

==> charts/precision_NORB.tex <==

\addplot[green] coordinates{
(100,1)
(150,1)
(200,1)
(250,1)
(300,1)
(400,1)
(500,1)
(600,0.979)
(700,0.93)
(800,0.9)
(900,0.877)
(1000,0.848)
(1500,0.755)
(2000,0.691)
(2500,0.656)
(3000,0.626)
(4000,0.59)
(5000,0.56)
(7500,0.517)
(10000,0.495)
(15000,0.43)
(20000,0.4122)
	};\label{plots:plot2}
\addplot[red] coordinates{
(100,1)
(150,1)
(200,1)
(250,1)
(300,1)
(400,1)
(500,1)
(600,1)
(700,1)
(800,1)
(900,1)
(1000,1)
(1500,0.963)
(2000,0.927)
(2500,0.876)
(3000,0.856)
(4000,0.81)
(5000,0.7796)
(7500,0.7422)
(10000,0.7)
(15000,0.6459)
(20000,0.6083)
};\label{plots:plot1}
\addplot[blue] coordinates{(100,0.77)
(150,0.657)
(200,0.54)
(250,0.473)
(300,0.438)
(400,0.381)
(500,0.366)
(600,0.333)
(700,0.3143)
(800,0.3)
(900,0.29)
(1000,0.28)
(1500,0.252)
(2000,0.2364)
(2500,0.22)
(3000,0.206)
(4000,0.195)
(5000,0.194)
(7500,0.179)
(10000,0.16)
(15000,0.1494)
(20000,0.1399)};\label{plots:plot3}
\addplot[black] coordinates{
(100,1)
(20000,1)
};\label{plots:plot4}

==> charts/precision_TIMIT.tex <==

\addplot[black] coordinates{
(100,1)
(200000,1)
	};\label{plots:plot1}
\addplot[red] coordinates{(100,1)
(150,1)
(200,1)
(250,1)
(300,1)
(400,1)
(500,1)
(600,1)
(700,1)
(800,1)
(1000,1)
(1500,0.999)
(2000,0.996)
(5000,0.974)
(7500,0.956)
(10000,0.947)
(15000,0.925)
(20000,0.9156)
(30000,0.9)
(50000,0.858)
(75000,0.839)
(100000,0.821)
(150000,0.808)
(200000,0.797)
};\label{plots:plot2}
\addplot[green] coordinates{(100,1)
(150,1)
(200,1)
(250,1)
(300,1)
(400,1)
(500,1)
(600,0.998)
(700,0.995)
(800,0.988)
(1000,0.977)
(1500,0.9468)
(2000,0.93)
(5000,0.86)
(7500,0.826)
(10000,0.8)
(15000,0.772)
(20000,0.747)
(30000,0.723)
(50000,0.676)
(75000,0.647)
(100000,0.636)
(150000,0.612)
(200000,0.599)};\label{plots:plot3}
\addplot[blue] coordinates{(100,0.815)
(150,0.743)
(200,0.663)
(250,0.6344)
(300,0.593)
(400,0.557)
(500,0.542)
(600,0.513)
(700,0.49)
(800,0.4855)
(1000,0.477)
(1500,0.445)
(2000,0.417)
(5000,0.3566)
(7500,0.334)
(10000,0.322)
(15000,0.2957)
(20000,0.285)
(30000,0.27)
(50000,0.247)
(75000,0.233)
(100000,0.225)
(150000,0.214)
(200000,0.207)};\label{plots:plot4}

==> charts/ratio_CIFAR.tex <==
\addplot[red] coordinates{(0,1.000)
(10,1.000)
(20,1.000)
(30,1.000)
(40,1.000)
(50,1.000)
(60,1.000)
(70,1.000)
(80,1.000)
(90,1.000)
(100,1.000)
(110,1.000)
(120,1.000)
(130,1.000)
(140,1.000)
(150,1.000)
(160,1.000)
(170,1.000)
(180,1.000)
(190,1.000)
(200,1.000)
(210,1.000)
(220,1.002)
(230,1.007)
(240,1.009)
(250,1.006)
(260,1.002)
(270,1.002)
(280,1.003)
(290,1.003)
(300,1.001)
(310,1.000)
(320,0.999)
(330,0.999)
(340,0.999)
(350,1.000)
(360,1.000)
(370,1.000)
(380,1.001)
(390,1.002)
(400,1.002)
(410,1.003)
(420,1.003)
(430,1.004)
(440,1.004)
(450,1.005)
(460,1.005)
(470,1.006)
(480,1.006)
(490,1.006)
(500,1.007)
(510,1.007)
(520,1.008)
(530,1.008)
(540,1.008)
(550,1.009)
(560,1.009)
(570,1.009)
(580,1.010)
(590,1.010)
(600,1.011)
(610,1.011)
(620,1.011)
(630,1.012)
(640,1.012)
(650,1.012)
(660,1.013)
(670,1.013)
(680,1.013)
(690,1.013)
(700,1.014)
(710,1.014)
(720,1.014)
(730,1.014)
(740,1.015)
(750,1.015)
(760,1.015)
(770,1.015)
(780,1.015)
(790,1.016)
(800,1.016)
(810,1.016)
(820,1.016)
(830,1.016)
(840,1.017)
(850,1.017)
(860,1.017)
(870,1.017)
(880,1.017)
(890,1.017)
(900,1.018)
(910,1.018)
(920,1.018)
(930,1.018)
(940,1.018)
(950,1.018)
(960,1.019)
(970,1.019)
(980,1.019)
(990,1.019)
(1000,1.019)
(1010,1.019)
(1020,1.020)
(1030,1.020)
(1040,1.020)
(1050,1.020)
(1060,1.020)
(1070,1.020)
(1080,1.021)
(1090,1.021)
(1100,1.021)
(1110,1.021)
(1120,1.021)
(1130,1.021)
(1140,1.021)
(1150,1.022)
(1160,1.022)
(1170,1.022)
(1180,1.022)
(1190,1.022)
(1200,1.022)
(1210,1.022)
(1220,1.023)
(1230,1.023)
(1240,1.023)
(1250,1.023)
(1260,1.023)
(1270,1.023)
(1280,1.023)
(1290,1.023)
(1300,1.023)
(1310,1.024)
(1320,1.024)
(1330,1.024)
(1340,1.024)
(1350,1.024)
(1360,1.024)
(1370,1.024)
(1380,1.024)
(1390,1.024)
(1400,1.025)
(1410,1.025)
(1420,1.025)
(1430,1.025)
(1440,1.025)
(1450,1.025)
(1460,1.025)
(1470,1.025)
(1480,1.025)
(1490,1.026)
(1500,1.026)
(1510,1.026)
(1520,1.026)
(1530,1.026)
(1540,1.026)
(1550,1.026)
(1560,1.026)
(1570,1.026)
(1580,1.026)
(1590,1.027)
(1600,1.027)
(1610,1.027)
(1620,1.027)
(1630,1.027)
(1640,1.027)
(1650,1.027)
(1660,1.027)
(1670,1.027)
(1680,1.027)
(1690,1.027)
(1700,1.028)
(1710,1.028)
(1720,1.028)
(1730,1.028)
(1740,1.028)
(1750,1.028)
(1760,1.028)
(1770,1.028)
(1780,1.028)
(1790,1.028)
(1800,1.028)
(1810,1.028)
(1820,1.029)
(1830,1.029)
(1840,1.029)
(1850,1.029)
(1860,1.029)
(1870,1.029)
(1880,1.029)
(1890,1.029)
(1900,1.029)
(1910,1.029)
(1920,1.029)
(1930,1.029)
(1940,1.029)
(1950,1.030)
(1960,1.030)
(1970,1.030)
(1980,1.030)
(1990,1.030)
(2000,1.030)
(2010,1.030)
(2020,1.030)
(2030,1.030)
(2040,1.030)
(2050,1.030)
(2060,1.030)
(2070,1.030)
(2080,1.031)
(2090,1.031)
(2100,1.031)
(2110,1.031)
(2120,1.031)
(2130,1.031)
(2140,1.031)
(2150,1.031)
(2160,1.031)
(2170,1.031)
(2180,1.031)
(2190,1.031)
(2200,1.031)
(2210,1.031)
(2220,1.031)
(2230,1.031)
(2240,1.031)
(2250,1.031)
(2260,1.031)
(2270,1.031)
(2280,1.031)
(2290,1.031)
(2300,1.031)
(2310,1.031)
(2320,1.031)
(2330,1.031)
(2340,1.031)
(2350,1.031)
(2360,1.031)
(2370,1.031)
(2380,1.031)
(2390,1.031)
(2400,1.031)
(2410,1.031)
(2420,1.031)
(2430,1.031)
(2440,1.031)
(2450,1.031)
(2460,1.031)
(2470,1.031)
(2480,1.031)
(2490,1.031)
(2500,1.031)};\label{plots:plot1}
\addplot[green] coordinates{(0,1.000)
(10,1.000)
(20,1.000)
(30,1.000)
(40,1.000)
(50,1.000)
(60,1.000)
(70,1.000)
(80,1.000)
(90,1.000)
(100,1.000)
(110,1.000)
(120,1.000)
(130,1.000)
(140,1.000)
(150,1.000)
(160,1.000)
(170,1.000)
(180,1.000)
(190,1.000)
(200,1.000)
(210,1.000)
(220,1.003)
(230,1.011)
(240,1.019)
(250,1.018)
(260,1.010)
(270,1.006)
(280,1.005)
(290,1.006)
(300,1.007)
(310,1.008)
(320,1.010)
(330,1.011)
(340,1.013)
(350,1.015)
(360,1.017)
(370,1.018)
(380,1.020)
(390,1.021)
(400,1.022)
(410,1.023)
(420,1.024)
(430,1.025)
(440,1.025)
(450,1.026)
(460,1.027)
(470,1.028)
(480,1.029)
(490,1.029)
(500,1.030)
(510,1.031)
(520,1.032)
(530,1.032)
(540,1.033)
(550,1.034)
(560,1.034)
(570,1.035)
(580,1.036)
(590,1.036)
(600,1.037)
(610,1.037)
(620,1.038)
(630,1.038)
(640,1.039)
(650,1.040)
(660,1.040)
(670,1.041)
(680,1.041)
(690,1.042)
(700,1.042)
(710,1.043)
(720,1.043)
(730,1.044)
(740,1.044)
(750,1.044)
(760,1.045)
(770,1.045)
(780,1.046)
(790,1.046)
(800,1.047)
(810,1.047)
(820,1.047)
(830,1.048)
(840,1.048)
(850,1.048)
(860,1.049)
(870,1.049)
(880,1.050)
(890,1.050)
(900,1.050)
(910,1.050)
(920,1.051)
(930,1.051)
(940,1.051)
(950,1.052)
(960,1.052)
(970,1.052)
(980,1.053)
(990,1.053)
(1000,1.053)
(1010,1.053)
(1020,1.054)
(1030,1.054)
(1040,1.054)
(1050,1.055)
(1060,1.055)
(1070,1.055)
(1080,1.055)
(1090,1.056)
(1100,1.056)
(1110,1.056)
(1120,1.056)
(1130,1.057)
(1140,1.057)
(1150,1.057)
(1160,1.058)
(1170,1.058)
(1180,1.058)
(1190,1.058)
(1200,1.059)
(1210,1.059)
(1220,1.059)
(1230,1.059)
(1240,1.059)
(1250,1.060)
(1260,1.060)
(1270,1.060)
(1280,1.060)
(1290,1.061)
(1300,1.061)
(1310,1.061)
(1320,1.061)
(1330,1.061)
(1340,1.062)
(1350,1.062)
(1360,1.062)
(1370,1.062)
(1380,1.062)
(1390,1.063)
(1400,1.063)
(1410,1.063)
(1420,1.063)
(1430,1.063)
(1440,1.064)
(1450,1.064)
(1460,1.064)
(1470,1.064)
(1480,1.064)
(1490,1.065)
(1500,1.065)
(1510,1.065)
(1520,1.065)
(1530,1.065)
(1540,1.065)
(1550,1.066)
(1560,1.066)
(1570,1.066)
(1580,1.066)
(1590,1.066)
(1600,1.066)
(1610,1.067)
(1620,1.067)
(1630,1.067)
(1640,1.067)
(1650,1.067)
(1660,1.067)
(1670,1.068)
(1680,1.068)
(1690,1.068)
(1700,1.068)
(1710,1.068)
(1720,1.068)
(1730,1.068)
(1740,1.069)
(1750,1.069)
(1760,1.069)
(1770,1.069)
(1780,1.069)
(1790,1.069)
(1800,1.069)
(1810,1.070)
(1820,1.070)
(1830,1.070)
(1840,1.070)
(1850,1.070)
(1860,1.070)
(1870,1.070)
(1880,1.070)
(1890,1.070)
(1900,1.071)
(1910,1.071)
(1920,1.071)
(1930,1.071)
(1940,1.071)
(1950,1.071)
(1960,1.071)
(1970,1.071)
(1980,1.071)
(1990,1.072)
(2000,1.072)
(2010,1.072)
(2020,1.072)
(2030,1.072)
(2040,1.072)
(2050,1.072)
(2060,1.072)
(2070,1.072)
(2080,1.072)
(2090,1.073)
(2100,1.073)
(2110,1.073)
(2120,1.073)
(2130,1.073)
(2140,1.073)
(2150,1.073)
(2160,1.073)
(2170,1.073)
(2180,1.073)
(2190,1.073)
(2200,1.073)
(2210,1.073)
(2220,1.073)
(2230,1.073)
(2240,1.073)
(2250,1.073)
(2260,1.074)
(2270,1.074)
(2280,1.074)
(2290,1.074)
(2300,1.074)
(2310,1.074)
(2320,1.074)
(2330,1.074)
(2340,1.074)
(2350,1.074)
(2360,1.074)
(2370,1.074)
(2380,1.074)
(2390,1.074)
(2400,1.074)
(2410,1.074)
(2420,1.074)
(2430,1.074)
(2440,1.074)
(2450,1.074)
(2460,1.074)
(2470,1.074)
(2480,1.074)
(2490,1.074)
(2500,1.074)};\label{plots:plot2}
\addplot[blue] coordinates{(0,1.000)
(10,1.000)
(20,1.000)
(30,1.000)
(40,1.000)
(50,1.000)
(60,1.000)
(70,1.000)
(80,1.000)
(90,1.000)
(100,1.000)
(110,1.000)
(120,1.000)
(130,1.000)
(140,1.000)
(150,1.000)
(160,1.000)
(170,1.000)
(180,1.000)
(190,1.000)
(200,1.000)
(210,1.000)
(220,1.003)
(230,1.012)
(240,1.023)
(250,1.032)
(260,1.094)
(270,1.134)
(280,1.087)
(290,1.061)
(300,1.050)
(310,1.044)
(320,1.043)
(330,1.045)
(340,1.047)
(350,1.050)
(360,1.053)
(370,1.056)
(380,1.059)
(390,1.062)
(400,1.065)
(410,1.067)
(420,1.070)
(430,1.072)
(440,1.074)
(450,1.076)
(460,1.078)
(470,1.080)
(480,1.082)
(490,1.084)
(500,1.086)
(510,1.087)
(520,1.089)
(530,1.091)
(540,1.092)
(550,1.094)
(560,1.095)
(570,1.097)
(580,1.098)
(590,1.100)
(600,1.101)
(610,1.102)
(620,1.104)
(630,1.105)
(640,1.106)
(650,1.108)
(660,1.109)
(670,1.110)
(680,1.111)
(690,1.112)
(700,1.113)
(710,1.114)
(720,1.116)
(730,1.117)
(740,1.118)
(750,1.119)
(760,1.120)
(770,1.121)
(780,1.122)
(790,1.123)
(800,1.124)
(810,1.125)
(820,1.125)
(830,1.126)
(840,1.127)
(850,1.128)
(860,1.129)
(870,1.130)
(880,1.131)
(890,1.131)
(900,1.132)
(910,1.133)
(920,1.134)
(930,1.135)
(940,1.135)
(950,1.136)
(960,1.137)
(970,1.138)
(980,1.138)
(990,1.139)
(1000,1.140)
(1010,1.141)
(1020,1.141)
(1030,1.142)
(1040,1.143)
(1050,1.143)
(1060,1.144)
(1070,1.145)
(1080,1.145)
(1090,1.146)
(1100,1.147)
(1110,1.147)
(1120,1.148)
(1130,1.148)
(1140,1.149)
(1150,1.150)
(1160,1.150)
(1170,1.151)
(1180,1.151)
(1190,1.152)
(1200,1.152)
(1210,1.153)
(1220,1.153)
(1230,1.154)
(1240,1.155)
(1250,1.155)
(1260,1.156)
(1270,1.156)
(1280,1.157)
(1290,1.157)
(1300,1.158)
(1310,1.158)
(1320,1.159)
(1330,1.159)
(1340,1.160)
(1350,1.160)
(1360,1.161)
(1370,1.161)
(1380,1.162)
(1390,1.162)
(1400,1.162)
(1410,1.163)
(1420,1.163)
(1430,1.164)
(1440,1.164)
(1450,1.165)
(1460,1.165)
(1470,1.166)
(1480,1.166)
(1490,1.167)
(1500,1.167)
(1510,1.167)
(1520,1.168)
(1530,1.168)
(1540,1.169)
(1550,1.169)
(1560,1.169)
(1570,1.170)
(1580,1.170)
(1590,1.171)
(1600,1.171)
(1610,1.171)
(1620,1.172)
(1630,1.172)
(1640,1.173)
(1650,1.173)
(1660,1.173)
(1670,1.174)
(1680,1.174)
(1690,1.174)
(1700,1.175)
(1710,1.175)
(1720,1.175)
(1730,1.176)
(1740,1.176)
(1750,1.176)
(1760,1.177)
(1770,1.177)
(1780,1.177)
(1790,1.178)
(1800,1.178)
(1810,1.178)
(1820,1.179)
(1830,1.179)
(1840,1.179)
(1850,1.179)
(1860,1.180)
(1870,1.180)
(1880,1.180)
(1890,1.181)
(1900,1.181)
(1910,1.181)
(1920,1.181)
(1930,1.182)
(1940,1.182)
(1950,1.182)
(1960,1.182)
(1970,1.183)
(1980,1.183)
(1990,1.183)
(2000,1.184)
(2010,1.184)
(2020,1.184)
(2030,1.184)
(2040,1.185)
(2050,1.185)
(2060,1.185)
(2070,1.185)
(2080,1.185)
(2090,1.186)
(2100,1.186)
(2110,1.186)
(2120,1.186)
(2130,1.187)
(2140,1.187)
(2150,1.187)
(2160,1.187)
(2170,1.187)
(2180,1.187)
(2190,1.188)
(2200,1.188)
(2210,1.188)
(2220,1.188)
(2230,1.188)
(2240,1.188)
(2250,1.189)
(2260,1.189)
(2270,1.189)
(2280,1.189)
(2290,1.189)
(2300,1.189)
(2310,1.189)
(2320,1.189)
(2330,1.190)
(2340,1.190)
(2350,1.190)
(2360,1.190)
(2370,1.190)
(2380,1.190)
(2390,1.190)
(2400,1.190)
(2410,1.190)
(2420,1.190)
(2430,1.190)
(2440,1.190)
(2450,1.191)
(2460,1.191)
(2470,1.191)
(2480,1.191)
(2490,1.191)
(2500,1.191)};\label{plots:plot3}


==> content/related_work_OLD.tex <==

\section{Related work}
\label{sec:related_work}

Interactive performance is at the center of the latest developments in Visual Analytics. New analytical tools and algorithms that are able to trade accuracy for speed and interactively refine results~\cite{FeketeOBB,TrustMe} are needed to deal with the scalability issues of existing analytics algorithms. M\"uhlbacher et al.~\cite{OpeningBlackBox} defined different strategies to increase the user involvement in existing algorithm implementation. They provide an in-depth analysis on how the interconnection between the visualization and the analytic modules can be achieved. Stolper et al.~\cite{progressiveVisualAnalytics} defined the term \emph{Progressive Visual Analytics} that describes techniques that allow the analyst to directly interact with the analytic process. Visualization of intermediate results is used to give the user clues on the data that can be used to change the parameters of the analytic algorithm or to filter the data. A guideline for the design of Progressive Visual Analytics is also provided. These works present theoretical frameworks but they do not consider that many algorithms are not directly suited for Progressive Visual Analytics. In our work, we present a Progressive Visual Analytics dimensionality reduction technique in which intermediate results can be quickly obtained thanks to the introduction of an approximation in the analytical process.\\

A first attempt in implementing a Progressive Visual Analytics can be found in the work from Jaegul Choo et al.~\cite{pive}. Based on the fact that most of the computational algorithms are iterative, they present a framework for the visualization and interaction with intermediate results. Two different types of interaction with the intermediate results are then presented: \emph{hard} and \emph{soft replacements}. In a \emph{soft replacement} the intermediate results can be changed by the user and the algorithm, whereas in a \emph{hard replacement} the intermediate results modified by the user cannot be changed by the algorithm afterwards.\\

In our work, we focus on dimensionality reduction algorithms for the visual analysis of high-dimensional spaces. We base our development on a machine learning algorithm, called tSNE~\cite{ref:tsne}, that aims at preserving local structures in the embedding, whilst showing also global information, such as the presence of clusters at several scales. This characteristic made tSNE widely used for the exploration and visualization of high-dimensional data ~\cite{visne,babcock2013deorphanizing,becher2014high,frome2013devise,decaf,
laczny2014alignment,mahfouz2014visualizing,AINature,ACCENSE}. tSNE's computational and memory complexity is $O(N^2)$, where $N$ is the number of data-points in the data, which constrains the application of the technique. An evolution of the algorithm, called Barnes-Hut-SNE (BH-SNE)~\cite{ref:bhtsne,LastFromLaurens}, reduces the computational complexity to $O(N \log(N) )$ and the memory complexity to $O(N)$. This approach was also developed in parallel by Zang et al.~\cite{ref:bhsne_2}.  However, despite the increased performance, it still cannot be used to interactively explore the data in a desktop environment. Even with a per-iteration visualization of the intermediate results~\cite{pive,OpeningBlackBox,progressiveVisualAnalytics}, the initialization time required to compute similarities in the high-dimensional space is too long. Changing parameters and the removal or the addition of points or dimensions will force the user to wait for the full reinitialization of the algorithm. This reinitialization requires minutes, or even hours, on a state of the art desktop computer.\\

We propose to compute an approximation of tSNE's preprocessing stage, followed by a user steerable~\cite{mulder1999survey} refinement. To compute the conditional probabilities needed by BH-SNE, a K-Nearest Neighborhood search (KNN) must be evaluated for each point in the high-dimensional space. Under these conditions a traditional algorithm and data structure, such as a KD-Tree~\cite{kdtree}, will not perform well. In the BH-SNE~\cite{ref:bhtsne} algorithm a Vantage-Point Tree~\cite{vptree} is used for the KNN search, but it is slow to query. In our work, an approximated computation of the KNN is used to achieve a compromise between quality and speed.\\

An approximated and user steerable dimensionality reduction algorithm is MDSteer~\cite{SteerableMDS}. MDSteer works on a subset of the data and allows the user to control the insertion of points by selecting areas in the reduced space. The technique presented by Yang et al.~\cite{yang2006fast} is based on dimensionality reduction algorithms in which a dissimilarity matrix is used as an input. By means of a divide-and-conquer approach, the computational complexity of the algorithms can be reduced. Other techniques are steerable in the sense that the dimensionality reduction is guided by user input~\cite{P0,P1,P2}. However they are not able to keep interaction with the whole space.\\

The visualization of the embedding by means of a scatterplot will be affected by visual clutter. Density-based visualization of the tSNE embedding has been used by several authors~\cite{visne,ACCENSE,LastFromLaurens}. In our work, we employed and improved a state-of-the-art technique~\cite{ref:KDE_Scatter_plots} for Kernel Density Estimation (KDE), that is suited for real-time visualization. The interaction with the embedding is important to allow the analyst to explore the high-dimensional data. Selection operations in the embedding and the visualization of the data in a coordinated multiple-view system are necessary to enable this exploration. The iVisClassifier system~\cite{ivisclassifier} is an example of such a solution. In our work we take a similar approach, providing a coordinated multiple-view framework for the visualization of a selection in the embedding.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
PDFFILES = paper.pdf
MAINTEXFILE = $(PDFFILES:.pdf=.tex)
SUBTEXFILES = 
BIBFILES = bibliography.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = pdflatex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg clean pdf

msg:
	@echo "   running latex compile"
	@echo ""

pdf:		$(PDFFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.pdf:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true
				open $(PDFFILES)
				osascript -e 'tell application "Preview" to activate'

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out *.tcp *.tps *.spl *.lbl $(PSFILES) *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

